Two ways towards combining Sequential Neural Network and Statistical Methods to Improve the Prediction of Time Series

Statistic modeling and data-driven learning are the two vital fields that attract many attentions. Statistic models intend to capture and interpret the relationships among variables, while data-based learning attempt to extract information directly from the data without pre-processing through complex models. Given the extensive studies in both fields, a subtle issue is how to properly integrate data based methods with existing knowledge or models. In this paper, based on the time series data, we propose two different directions to integrate the two, a decomposition-based method and a method exploiting the statistic extraction of data features. The first one decomposes the data into linear stable, nonlinear stable and unstable parts, where suitable statistical models are used for the linear stable and nonlinear stable parts while the appropriate machine learning tools are used for the unstable parts. The second one applies statistic models to extract statistics features of data and feed them as additional inputs into the machine learning platform for training. The most critical and challenging thing is how to determine and extract the valuable information from mathematical or statistical models to boost the performance of machine learning algorithms. We evaluate the proposal using time series data with varying degrees of stability. Performance results show that both methods can outperform existing schemes that use models and learning separately, and the improvements can be over 60%. Both our proposed methods are promising in bridging the gap between model-based and data-driven schemes and integrating the two to provide an overall higher learning performance.

==> Data2nd.tex <==
\subsection{Data-driven \del{Learning}\rev{Neural Networks}}
\vspace{-0.10in}
In modern machine learning and deep learning methods, rather than following a pre-established model, knowledge is directly derived from the data with \rev{various types of neural networks}.  
%Taking deep supervised learning as an example, it mainly starts from the data itself, sets the corresponding activation function and loss function, and passes the given input and output during the training phase. 
\rev{Although this method does not make assumption on the data distribution format and can} well follow nonlinear data, it suffers from large computational cost, weak interpretability,  \rev{and bias when  data  are unbalanced.} In the case of time series, the sequential neural networks, such as Recurrent Neural Network (RNN)\cite{madan2018predicting}, Long Short-Term Memory (LSTM)\cite{reddy2018prediction} and Gated Recurrent Units (GRU)\cite{fu2016using}, are often applied. 
\paragraph{Recurrent Neural Network}
\vspace{-0.10in}

\begin{figure}
%  \vspace{-25pt}
  \begin{center}
\includegraphics[width=2.5 in]{images/RNN.png}
  \end{center}
  \vspace{-10pt}
  \caption{\footnotesize RNN Structure}
\label{RNN}
  \vspace{-10pt}
%\end{wrapfigure}
\end{figure}


RNN \del{includes a  neural network that} can provide a very straight-forward but effective way of handling time series or other sequential data. \rv{As shown in Fig~\ref{RNN}, RNN follows a recurrent structure,} where the same function is performed for each time stage and the output of the previous time stage is the input of the next stage.  Given the sequence of input x = (x1,...xt), RNN iteratively calculates  \rev{the vector $h^* = (h^*_1;...; h^*_t)$ of the hidden layer and  $y = (y_1;...; y_t)$ of the output layer \del{for $t = 1$ to $T $} as follows }:
\begin{equation}
     h^*_t = H(W_{xh^*}x_t + W_{h^*h^*}h^*_{t-1}+b_h^*), \hspace{0.05in}  y_t = W_{h^*y}h^*_t + b_y,
\end{equation}
%\begin{equation}
%    y_t = W_{hy}h_t + b_y
%\end{equation}
where  $h^*_t$ is the  hidden vector,  $b_h^*$ is the hidden bias, $H$ is the hidden layer function, $W_{h^*h^*}$ is the weight at previous hidden state and $W_{xh^*}$ is the weight at the current state, $y_t$ is the output state, $W_{h^*y}$ is the weight at the current hidden state and $b_y$ is the output bias. RNN can model a sequence of data so that each sample \del{can be assumed to be dependent on} \rev{depends on} previous ones. Backward Propagation Algorithm is often used to train RNN. 

%\begin{wrapfigure}[10]{r}{2.5in}

\paragraph{Long Short-Term Memory}
\vspace{-0.15in}

\begin{figure}
%\begin{wrapfigure}[10]{r}{2.5in}
%  \vspace{-45pt}
  \begin{center}
\includegraphics[width=2.5 in]{images/LSTM.png}
  \end{center}
  \vspace{-10pt}
  \caption{\footnotesize Basic LSTM Structure}
\label{LSTM}
  \vspace{-10pt}
\end{figure}

RNN cannot process very long sequences, because \rev{the} back-propagated error  either explodes or vanishes \del{during the propagation} in the training process.  To alleviate the problem, 
LSTM is introduced. 
%Simply put, LSTM can perform better in longer sequences than normal RNN.
LSTM has two transmission states, the  cell state $c_t$  and the hidden state $h^*_t$. $c_t$  changes slowly, while $h^*_t$ changes faster. 
Fig~\ref{LSTM} shows the structure of LSTM with a single layer cell. \note {Temporal layer to spatial layer?} 
An LSTM layer \note{temporal or spatial layer?} consists of many \rev{recurrent}
memory cells and each cell contains three multiplicative gate units, \rev{{\em input,
forget and output.}} An LSTM architecture \rev{can be expressed with} the following composite functions:
\begin{equation}
    i_t = \sigma(W_{xi}x_t + W_{h^*i}h^*_t-1 + b_i), \hspace{0.1in}  f_t = \sigma(W_{xf}x_t + W_{h^*f}h^*_{t-1} + b_f), \hspace{0.1in} \mbox{and}  \hspace{0.1in} o_t = \sigma(W_{xo}x_t + W_{h^*o}h^*_{t^*-1}+b_o)
\end{equation}


%\begin{equation}
%    f_t = \sigma(W_{xf}x_t + W_{hf}h_{t-1} + b_f)
%\end{equation}
\begin{equation}
    c_t = f_tc_{t-1} + i_ttanh(W_{xc}x_t + W_{h^*c}h^*_{t-1}+b_c), \hspace{0.1in} \mbox{and}  \hspace{0.1in}  h^*_t = o_ttanh(c_t). 
\end{equation}
%\begin{equation}
%    o_t = \sigma(W_{xo}x_t + W_{ho}h_{t-1}+b_o)
%\end{equation}
%\begin{equation}
%    h_t = o_ttanh(c_t)
%\end{equation}
where $\sigma$ is the logistic sigmoid function, and $i$, $f$, $o$ and $c$ stand for input gates, forget gates, output gates and cell vectors. In LSTM, weights are divided into 3 sets, input weights ($W_{xi}$, $W_{xf}$, $W_{xc}$, $W_{xo}$ $\in{R^{N \times M}}$), recurrent weights ($W_{h^*i}$,$W_{h^*f}$ ,$W_{h^*c}$,$W_{h^*o}$ $\in{R^{N \times N}}$) and bias weights ($b_i$,$b_f$,$b_c$,$b_o$ $\in{R^N}$).  $N$ is the number of LSTM cells, and $M$ is the dimension of the input.
\note{Format your equation. It does not see that each row cannot hold two.}

==> Experiment_3rd.tex <==
\section{Experiment Analysis}
\subsection{Data Prepossessing}
Fig 1 shows the daily open stock price for "Federal Home Loan Mortgage Corp(FMCC)" Company from 01-02-2018 to 11-02-2018. In the very beginning, the stationary of this series should be checked since it's the requirement to build up the time related statistical model. Augmented Dickey-Fuller Test(ADF) test and KPSS test are the most popular method to check the stationary of the time series. The null hypothesis for ADF test is the time series is not stationary while the null hypothesis for KPSS is the time series is stationary. Table 1 and table 2 show the ADF and KPSS test results. From the P-value in Table, we should accept the null hypothesis of ADF test and reject the null hypothesis of KPSS test and conclude the time series is not stationary at the 5 percent level of significance.
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{5}{|l|}{Table 1: ADF Test Results for Open Price}                 \\ \hline
\multicolumn{3}{|l|}{Dickey-Fuller}          & \multicolumn{2}{l|}{-1.9106}    \\ \hline
\multicolumn{3}{|l|}{P-value}                & \multicolumn{2}{l|}{0.6135}     \\ \hline
\multicolumn{3}{|l|}{Null hypothesis} & \multicolumn{2}{l|}{Non-stationary} \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{5}{|l|}{Table 2: KPSS Test Results for Open Price}         \\ \hline
\multicolumn{3}{|l|}{KPSS Level}      & \multicolumn{2}{l|}{2.2152}     \\ \hline
\multicolumn{3}{|l|}{P-value}         & \multicolumn{2}{l|}{0.01}       \\ \hline
\multicolumn{3}{|l|}{Null hypothesis} & \multicolumn{2}{l|}{Stationary} \\ \hline
\end{tabular}
\end{table}
Next, the key becomes how to transfer the unstationry data into stationary one. There are many different methods can be used to make the data more stationary like logarithm, difference, Power transform, etc. Here we use the most popular one-difference to transform the data. Fig 2 shows the differences data of the original time series.Further, the stationary will be checked again to ensure that the data is stable after the difference. Table 3 and table 4 show the ADF and KPSS test results. From the p-values in table 2, one can conclude that the differenced data is stationary now. 

\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{5}{|l|}{Table 3: ADF Test Results for Open Price}              \\ \hline
\multicolumn{3}{|l|}{Dickey-Fuller}   & \multicolumn{2}{l|}{-6.6027}        \\ \hline
\multicolumn{3}{|l|}{P-value}         & \multicolumn{2}{l|}{0.01}           \\ \hline
\multicolumn{3}{|l|}{Null hypothesis} & \multicolumn{2}{l|}{Non-stationary} \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{5}{|l|}{Table 4: KPSS Test Results for Open Price}         \\ \hline
\multicolumn{3}{|l|}{KPSS Level}      & \multicolumn{2}{l|}{0.36596}    \\ \hline
\multicolumn{3}{|l|}{P-value}         & \multicolumn{2}{l|}{0.092}      \\ \hline
\multicolumn{3}{|l|}{Null hypothesis} & \multicolumn{2}{l|}{Stationary} \\ \hline
\end{tabular}
\end{table}

\subsection{ARIMA-GARCH Model}
\subsubsection{ARIMA Model Selection}

When the series are stationary, the next step is to build up a appropriate ARIMA model for it. ACF and PACF plots will be helpful to make selection for ARIMA model, which are shown in fig 3. From the ACF and PACF plots, we do see the auto-correlation and partial auto-correlation in the time series. However, to make a more accurate model, we use the auto.arima function in R studio to make the exact selection. The auto.arima function in R studio will select the model  based on either the AIC, BIC or AICc. Fig 4 shows the result of auto.arima. So far, ARIMA(5,0,2) will be used to model the differenced time series. The Table 3 below shows the result of ARIMA(5,0,2) model. 
\begin{table}[]
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\multicolumn{6}{|c|}{Table 5: Results of ARIMA Model} \\ \hline
 & ar1 & ar2 & ar3 & ar4 & ar5 \\ \hline
Coefficients of AR & -0.618 & -0.3506 & -0.0379 & 0.0299 & 0.1604 \\ \hline
standard errors & \multicolumn{1}{l|}{0.471} & \multicolumn{1}{l|}{0.4322} & \multicolumn{1}{l|}{0.1109} & \multicolumn{1}{l|}{0.1000} & \multicolumn{1}{l|}{0.0835} \\ \hline
 & \multicolumn{3}{c|}{ma1} & \multicolumn{2}{c|}{ma2} \\ \hline
Coefficients of MA & \multicolumn{3}{c|}{0.5223} & \multicolumn{2}{c|}{0.1836} \\ \hline
standard errors & \multicolumn{3}{c|}{0.4800} & \multicolumn{2}{c|}{0.4469} \\ \hline
AIC & \multicolumn{5}{c|}{-593.7} \\ \hline
\end{tabular}
\end{table}
\subsubsection{ARIMA Model Diagnostic Test}
The significance test of the model is mainly to test the validity of the model.The residuals for a good model should not contain any correlation information,that is, the residuals should be the white noise; Otherwise, the model is not valid and other models should be reconsidered. Ljung-Box test is a powerful tool to test the white noise. The null hypothesis of this test is the tested series is a white noise while the alternative hypothesis is the series is not a white noise. The table below shows the Ljung-Box test result, from which one can not reject the null hypothesis and conclude that the ARIMA(5,0,2) model is valid.

\begin{table}[]
\centering
\begin{tabular}{|c|l|l|c|l|}
\hline
\multicolumn{5}{|c|}{\begin{tabular}[c]{@{}c@{}} Table 6: Ljung-Box Diagnostic Test   \\    Results for ARIMA Model \end{tabular}} \\ \hline
\multicolumn{3}{|c|}{Lag} & \multicolumn{2}{c|}{P-value} \\ \hline
\multicolumn{3}{|c|}{2} & \multicolumn{2}{c|}{0.9497} \\ \hline
\multicolumn{3}{|c|}{4} & \multicolumn{2}{c|}{0.9762} \\ \hline
\multicolumn{3}{|c|}{6} & \multicolumn{2}{c|}{0.9906} \\ \hline
\multicolumn{3}{|c|}{8} & \multicolumn{2}{c|}{0.9945} \\ \hline
\multicolumn{3}{|c|}{10} & \multicolumn{2}{c|}{0.9989} \\ \hline
\multicolumn{3}{|c|}{12} & \multicolumn{2}{c|}{0.9998} \\ \hline
\multicolumn{3}{|c|}{14} & \multicolumn{2}{c|}{0.9954} \\ \hline
\multicolumn{3}{|c|}{16} & \multicolumn{2}{c|}{0.9984} \\ \hline
\multicolumn{3}{|c|}{18} & \multicolumn{2}{c|}{0.9987} \\ \hline
\multicolumn{3}{|c|}{20} & \multicolumn{2}{c|}{0.9987} \\ \hline
\end{tabular}
\end{table}

\subsubsection{ARCH Effect Test}
ARCH effect measures the fluctuation of time series. After the model passes the test, there is no correlation between the residuals themselves but the relationship between the changes in the residuals needs to be considered. In other words,  the homogeneity of variance in the residuals should be take into account. Fortunately, the homogeneity test of variance can be converted to the autocorrelation test of the residual square sequence. Therefore, the Lagrange Multiplier(LM) test method is used to test the autocorrelation of the residual square sequence, to simply find whether there is the ARCH effect in the residual sequence. The null hypothesis of the LM test is that the variance of the residual square sequence is homogeneous. Table x shows the result of LM test, from which one can reject the null hypothesis and conclude there is arch effect in the residual sequence. Then GARCH model should be used next. 
\begin{table}[]
\centering
\begin{tabular}{|c|l|l|c|l|}
\hline
\multicolumn{5}{|c|}{\begin{tabular}[c]{@{}c@{}}Table 7: Ljung-Box Arch Effect Test \\ Results for  Residuals\end{tabular}} \\ \hline
\multicolumn{3}{|c|}{Lag} & \multicolumn{2}{c|}{P-value} \\ \hline
\multicolumn{3}{|c|}{2} & \multicolumn{2}{c|}{9.992e-16} \\ \hline
\multicolumn{3}{|c|}{4} & \multicolumn{2}{c|}{2.753e-14} \\ \hline
\multicolumn{3}{|c|}{6} & \multicolumn{2}{c|}{4.745e-13} \\ \hline
\multicolumn{3}{|c|}{8} & \multicolumn{2}{c|}{3.561e-12} \\ \hline
\multicolumn{3}{|c|}{10} & \multicolumn{2}{c|}{2.579e-11} \\ \hline
\multicolumn{3}{|c|}{12} & \multicolumn{2}{c|}{1.178e-10} \\ \hline
\multicolumn{3}{|c|}{14} & \multicolumn{2}{c|}{6.767e-10} \\ \hline
\multicolumn{3}{|c|}{16} & \multicolumn{2}{c|}{2.105e-09} \\ \hline
\multicolumn{3}{|c|}{18} & \multicolumn{2}{c|}{8.386e-09} \\ \hline
\multicolumn{3}{|c|}{20} & \multicolumn{2}{c|}{3.15e-08} \\ \hline
\end{tabular}
\end{table}

\subsubsection{Building Up ARIMA-GARCH Model}
GARCH part model selection is based on AIC. The table below display all the AIC value for P&Q from 1 to 5. From table x, we finally select ARIMA(5,0,2)-GARCH(1,1) model since this model has the smallest AIC. The specific model information is shown in equation x. 

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multicolumn{6}{|l|}{Table 8: Arima(5,0,2)-Garch(p,q) order selection} \\ \hline
    & 1           & 2           & 3          & 4          & 5          \\ \hline
1   & -3.144827   & -3.112094   & -3.114695  & -3.080765  & -3.047413  \\ \hline
2   & -3.132756   & -3.107489   & -3.089428  & -3.055498  & -3.022146  \\ \hline
3   & -3.102736   & -3.077602   & -3.064161  & -3.030231  & -2.996879  \\ \hline
4   & -3.070756   & -3.045544   & -3.030231  & -3.004964  & -2.971612  \\ \hline
5   & -3.048537   & -3.023396   & -3.004462  & -2.979283  & -2.954017  \\ \hline
\end{tabular}
\end{table}
\subsubsection{ARIMA-GARCH Model Diagnostic Test}
After build up the ARIMA(5,0,2)-GARCH(1,1) model, we still need to check the validity of the model. Ljung-Box test will be used to test whether the residuals here is white noise and Lagrange Multiplier test will be used to check the arch effect of the residuals. Table X shows the  results for both of the tests, from which one can conclude ARIMA(5,0,2)-GARCH(1,1) model is valid and all the arch effect is deleted.
\begin{table}[]
\centering
\begin{tabular}{|l|l|}
\hline
\multicolumn{2}{|l|}{\begin{tabular}[c]{@{}l@{}}Table 9: Ljung-Box Diagnostic Test\\ Results for ARIMA-GARCH Model\end{tabular}} \\ \hline
Lag & P-value \\ \hline
2   & 0.9409  \\ \hline
4   & 0.8442  \\ \hline
6   & 0.2973  \\ \hline
8   & 0.2289  \\ \hline
10  & 0.3505  \\ \hline
12  & 0.5196  \\ \hline
14  & 0.4261  \\ \hline
16  & 0.5607  \\ \hline
18  & 0.6848  \\ \hline
20  & 0.7812  \\ \hline
\end{tabular}
\end{table}
\subsection{Results analysis of decomposition based method}
According to the ARIMA-GARCH model above, one can get the unstable part $N_t$ by $N_t = y_t - ARIMA(5,0,2)-GARCH(1,1)$. Next, ML models are used to deal with $N_t$. To predict the future, we will make both one-step and multi-steps predictions. The results below show the comparisons among ARIMA-GARCH-SVR, ARIMA-GARCH-LSTM, SVR, LSTM and ARIMA-GARCH, from which one can see ARIM-GARCH-SVR model has the best performance. Figure~\ref{PreM1}

\begin{wrapfigure}
  \vspace{5pt}
  \begin{center}
\includegraphics[width=2.5 in]{images/Predictions_M1.png}
  \end{center}
  \vspace{-20pt}
  \caption{\footnotesize Open Price Predictions of Different Methods}
\label{PreM1}
  \vspace{10pt}
\end{wrapfigure}

%[12]{r}{2.5in}
\begin{wrapfigure}
  \vspace{5pt}
  \begin{center}
\includegraphics[width=2.5 in]{images/MSEs_M1.png}
  \end{center}
  \vspace{-20pt}
  \caption{\footnotesize MSEs}
\label{MseM1}
  \vspace{20pt}
\end{wrapfigure}

%[12]{r}{2.5in}
\begin{wrapfigure}
  \vspace{5pt}
  \begin{center}
\includegraphics[width=2.5 in]{images/RollingM1.png}
  \end{center}
  \vspace{-20pt}
  \caption{\footnotesize Multiple Steps Predictions of Open Price}
\label{Rolling}
  \vspace{20pt}
\end{wrapfigure}

\begin{wrapfigure}
  \vspace{5pt}
  \begin{center}
\includegraphics[width=2.5 in]{images/RollingMse.png}
  \end{center}
  \vspace{-20pt}
  \caption{\footnotesize MSEs of Different Prediction Steps}
\label{RollingMse}
  \vspace{20pt}
\end{wrapfigure}


\subsection{Results analysis of statistics extraction based method}

First, the original data will be modeled as a comparison. A "Many input to many output" LSTM is trained with epochs 100 to make next 10 steps prediction. The parameter of look back size changing from 10 to 50 with step of 5. The results come from training stage show look back size of 40 will have the lowest training losses. Then, the extract the statistic $h_t$ will be added as a new variable with the past values of $y_t$ into LSTM. The training results show the look back size of 40 is the best choice. Figure X shows the  profiles of predicted values of LSTM with solo $y_t$ as input, of LSTM with $y_t$ and $h_t$ and the true values. And the table X1 gives the MSE of the two LSTM prediction results. 


%there are two different algorithms: rolling algorithm and non-rolling algorithm. The rolling method will keep adding the next test data into the training set and only make 1 step prediction each time;while the non-rolling method just based on the original training set and make multi-steps prediction.




































==> Experiment_Analysis.tex <==
\section{Experiment Analysis}


\note{You need to describe experiment set up first. Also what data set you use give references., and why you choose these. What reference work you use as comparison, why you choose them etc. 
Check how people writ this paper. Without these basic introductions, the paper is not readable.  }
\subsection{Data Prepossessing}
Fig 1 shows the daily open stock price for "Federal Home Loan Mortgage Corp(FMCC)" Company from 01-02-2018 to 11-02-2018. In the very beginning, the stationary of this series should be checked since it's the requirement to build up the time related statistical model. Augmented Dickey-Fuller Test(ADF) test and KPSS test are the most popular method to check the stationary of the time series. The null hypothesis \note{What is null hyo?} for ADF test is the time series is not stationary \note{not readable sentence.} while the null hypothesis for KPSS is the time series is stationary. \note{Another not readable wrong grammar sentence?} Table 1 and table 2 show the ADF and KPSS test results. From the P-value in Table, we should accept the null hypothesis of ADF test and reject the null hypothesis of KPSS test and conclude the time series is not stationary at the 5 percent level of significance.

\note{Why the stationary analysis related to this work? } 
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{5}{|l|}{Table 1: ADF Test Results for Open Price}                 \\ \hline
\multicolumn{3}{|l|}{Dickey-Fuller}          & \multicolumn{2}{l|}{-1.9106}    \\ \hline
\multicolumn{3}{|l|}{P-value}                & \multicolumn{2}{l|}{0.6135}     \\ \hline
\multicolumn{3}{|l|}{Null hypothesis} & \multicolumn{2}{l|}{Non-stationary} \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{5}{|l|}{Table 2: KPSS Test Results for Open Price}         \\ \hline
\multicolumn{3}{|l|}{KPSS Level}      & \multicolumn{2}{l|}{2.2152}     \\ \hline
\multicolumn{3}{|l|}{P-value}         & \multicolumn{2}{l|}{0.01}       \\ \hline
\multicolumn{3}{|l|}{Null hypothesis} & \multicolumn{2}{l|}{Stationary} \\ \hline
\end{tabular}
\end{table}
Next, the key becomes how to transfer the unstationry data into stationary one. \note{why do you want to translate to stationary one? Doesn't this change the data?} There are many different methods can be used to make the data more stationary like logarithm, difference, Power transform, etc. Here we use the most popular one-difference to transform the data. Fig 2 shows the differences data of the original time series.Further, the stationary will be checked again to ensure that the data is stable after the difference. Table 3 and table 4 show the ADF and KPSS test results. From the p-values in table 2, one can conclude that the differenced data is stationary now.  \note{isn't our purpose to model better dynamic data? Why changing them to stationary?}

\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{5}{|l|}{Table 3: ADF Test Results for Open Price}              \\ \hline
\multicolumn{3}{|l|}{Dickey-Fuller}   & \multicolumn{2}{l|}{-6.6027}        \\ \hline
\multicolumn{3}{|l|}{P-value}         & \multicolumn{2}{l|}{0.01}           \\ \hline
\multicolumn{3}{|l|}{Null hypothesis} & \multicolumn{2}{l|}{Non-stationary} \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{5}{|l|}{Table 4: KPSS Test Results for Open Price}         \\ \hline
\multicolumn{3}{|l|}{KPSS Level}      & \multicolumn{2}{l|}{0.36596}    \\ \hline
\multicolumn{3}{|l|}{P-value}         & \multicolumn{2}{l|}{0.092}      \\ \hline
\multicolumn{3}{|l|}{Null hypothesis} & \multicolumn{2}{l|}{Stationary} \\ \hline
\end{tabular}
\end{table}

\subsection{ARIMA-GARCH Model}
\subsubsection{ARIMA Model Selection}

When the series are stationary, \note{what if they are not stationary?} the next step is to build up a appropriate ARIMA model for it. ACF and PACF plots will be helpful to make selection for ARIMA model, which are shown in fig 3. From the ACF and PACF plots, \note{what are these plots?} we do see the auto-correlation and partial auto-correlation in the time series. However, to make a more accurate model, we use the auto.arima function in R studio to make the exact selection. The auto.arima function in R studio will select the model  based on either the AIC, BIC or AICc. Fig 4 shows the result of auto.arima. So far, ARIMA(5,0,2) will be used to model the differenced time series. The Table 3 below shows the result of ARIMA(5,0,2) model. \note{Don't assume that people have statistics knowledge. This whole writing seems to come from nowhere. How are they related to our current work? The change of data makes this work not trustable. }


\note{You are expected to compare the performance of these different models, in different set up. Why are you describing each model test? It is so weird. I am not sure you have been doing the right things.}

\begin{table}[]
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\multicolumn{6}{|c|}{Table 5: Results of ARIMA Model} \\ \hline
 & ar1 & ar2 & ar3 & ar4 & ar5 \\ \hline
Coefficients of AR & -0.618 & -0.3506 & -0.0379 & 0.0299 & 0.1604 \\ \hline
standard errors & \multicolumn{1}{l|}{0.471} & \multicolumn{1}{l|}{0.4322} & \multicolumn{1}{l|}{0.1109} & \multicolumn{1}{l|}{0.1000} & \multicolumn{1}{l|}{0.0835} \\ \hline
 & \multicolumn{3}{c|}{ma1} & \multicolumn{2}{c|}{ma2} \\ \hline
Coefficients of MA & \multicolumn{3}{c|}{0.5223} & \multicolumn{2}{c|}{0.1836} \\ \hline
standard errors & \multicolumn{3}{c|}{0.4800} & \multicolumn{2}{c|}{0.4469} \\ \hline
AIC & \multicolumn{5}{c|}{-593.7} \\ \hline
\end{tabular}
\end{table}
\subsubsection{ARIMA Model Diagnostic Test}
The significance test of the model is mainly to test the validity of the model.The residuals for a good model should not contain any correlation information,that is, the residuals should be the white noise; Otherwise, the model is not valid and other models should be reconsidered. Ljung-Box test is a powerful tool to test the white noise. The null hypothesis of this test is the tested series is a white noise while the alternative hypothesis is the series is not a white noise. The table below shows the Ljung-Box test result, from which one can not reject the null hypothesis and conclude that the ARIMA(5,0,2) model is valid.

\begin{table}[]
\centering
\begin{tabular}{|c|l|l|c|l|}
\hline
\multicolumn{5}{|c|}{\begin{tabular}[c]{@{}c@{}} Table 6: Ljung-Box Diagnostic Test   \\    Results for ARIMA Model \end{tabular}} \\ \hline
\multicolumn{3}{|c|}{Lag} & \multicolumn{2}{c|}{P-value} \\ \hline
\multicolumn{3}{|c|}{2} & \multicolumn{2}{c|}{0.9497} \\ \hline
\multicolumn{3}{|c|}{4} & \multicolumn{2}{c|}{0.9762} \\ \hline
\multicolumn{3}{|c|}{6} & \multicolumn{2}{c|}{0.9906} \\ \hline
\multicolumn{3}{|c|}{8} & \multicolumn{2}{c|}{0.9945} \\ \hline
\multicolumn{3}{|c|}{10} & \multicolumn{2}{c|}{0.9989} \\ \hline
\multicolumn{3}{|c|}{12} & \multicolumn{2}{c|}{0.9998} \\ \hline
\multicolumn{3}{|c|}{14} & \multicolumn{2}{c|}{0.9954} \\ \hline
\multicolumn{3}{|c|}{16} & \multicolumn{2}{c|}{0.9984} \\ \hline
\multicolumn{3}{|c|}{18} & \multicolumn{2}{c|}{0.9987} \\ \hline
\multicolumn{3}{|c|}{20} & \multicolumn{2}{c|}{0.9987} \\ \hline
\end{tabular}
\end{table}

\subsubsection{ARCH Effect Test}
ARCH effect measures the fluctuation of time series. After the model passes the test, there is no correlation between the residuals themselves but the relationship between the changes in the residuals needs to be considered. In other words,  the homogeneity of variance in the residuals should be take into account. Fortunately, the homogeneity test of variance can be converted to the autocorrelation test of the residual square sequence. Therefore, the Lagrange Multiplier(LM) test method is used to test the autocorrelation of the residual square sequence, to simply find whether there is the ARCH effect in the residual sequence. The null hypothesis of the LM test is that the variance of the residual square sequence is homogeneous. Table x shows the result of LM test, from which one can reject the null hypothesis and conclude there is arch effect in the residual sequence. Then GARCH model should be used next. 
\begin{table}[]
\centering
\begin{tabular}{|c|l|l|c|l|}
\hline
\multicolumn{5}{|c|}{\begin{tabular}[c]{@{}c@{}}Table 7: Ljung-Box Arch Effect Test \\ Results for  Residuals\end{tabular}} \\ \hline
\multicolumn{3}{|c|}{Lag} & \multicolumn{2}{c|}{P-value} \\ \hline
\multicolumn{3}{|c|}{2} & \multicolumn{2}{c|}{9.992e-16} \\ \hline
\multicolumn{3}{|c|}{4} & \multicolumn{2}{c|}{2.753e-14} \\ \hline
\multicolumn{3}{|c|}{6} & \multicolumn{2}{c|}{4.745e-13} \\ \hline
\multicolumn{3}{|c|}{8} & \multicolumn{2}{c|}{3.561e-12} \\ \hline
\multicolumn{3}{|c|}{10} & \multicolumn{2}{c|}{2.579e-11} \\ \hline
\multicolumn{3}{|c|}{12} & \multicolumn{2}{c|}{1.178e-10} \\ \hline
\multicolumn{3}{|c|}{14} & \multicolumn{2}{c|}{6.767e-10} \\ \hline
\multicolumn{3}{|c|}{16} & \multicolumn{2}{c|}{2.105e-09} \\ \hline
\multicolumn{3}{|c|}{18} & \multicolumn{2}{c|}{8.386e-09} \\ \hline
\multicolumn{3}{|c|}{20} & \multicolumn{2}{c|}{3.15e-08} \\ \hline
\end{tabular}
\end{table}

\subsubsection{Building Up ARIMA-GARCH Model}
GARCH part model selection is based on AIC. The table below display all the AIC value for P&Q from 1 to 5. From table x, we finally select ARIMA(5,0,2)-GARCH(1,1) model since this model has the smallest AIC. The specific model information is shown in equation x. 

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multicolumn{6}{|l|}{Table 8: Arima(5,0,2)-Garch(p,q) order selection} \\ \hline
    & 1           & 2           & 3          & 4          & 5          \\ \hline
1   & -3.144827   & -3.112094   & -3.114695  & -3.080765  & -3.047413  \\ \hline
2   & -3.132756   & -3.107489   & -3.089428  & -3.055498  & -3.022146  \\ \hline
3   & -3.102736   & -3.077602   & -3.064161  & -3.030231  & -2.996879  \\ \hline
4   & -3.070756   & -3.045544   & -3.030231  & -3.004964  & -2.971612  \\ \hline
5   & -3.048537   & -3.023396   & -3.004462  & -2.979283  & -2.954017  \\ \hline
\end{tabular}
\end{table}
\subsubsection{ARIMA-GARCH Model Diagnostic Test}
After build up the ARIMA(5,0,2)-GARCH(1,1) model, we still need to check the validity of the model. Ljung-Box test will be used to test whether the residuals here is white noise and Lagrange Multiplier test will be used to check the arch effect of the residuals. Table X shows the  results for both of the tests, from which one can conclude ARIMA(5,0,2)-GARCH(1,1) model is valid and all the arch effect is deleted.
\begin{table}[]
\centering
\begin{tabular}{|l|l|}
\hline
\multicolumn{2}{|l|}{\begin{tabular}[c]{@{}l@{}}Table 9: Ljung-Box Diagnostic Test\\ Results for ARIMA-GARCH Model\end{tabular}} \\ \hline
Lag & P-value \\ \hline
2   & 0.9409  \\ \hline
4   & 0.8442  \\ \hline
6   & 0.2973  \\ \hline
8   & 0.2289  \\ \hline
10  & 0.3505  \\ \hline
12  & 0.5196  \\ \hline
14  & 0.4261  \\ \hline
16  & 0.5607  \\ \hline
18  & 0.6848  \\ \hline
20  & 0.7812  \\ \hline
\end{tabular}
\end{table}
\subsection{Results analysis of decomposition based method}
According to the ARIMA-GARCH model above, one can get the unstable part $N_t$ by $N_t = y_t - ARIMA(5,0,2)-GARCH(1,1)$. Next, ML models are used to deal with $N_t$. To predict the future, we will make both one-step and multi-steps predictions. The results below show the comparisons among ARIMA-GARCH-SVR, ARIMA-GARCH-LSTM, SVR, LSTM and ARIMA-GARCH, from which one can see ARIM-GARCH-SVR model has the best performance. 




\subsection{Results analysis of statistics extraction based method}

First, the original data will be modeled as a comparison. A "Many input to many output" LSTM is trained with epochs 100 to make next 10 steps prediction. The parameter of look back size changing from 10 to 50 with step of 5. The results come from training stage show look back size of 40 will have the lowest training losses. Then, the extract the statistic $h_t$ will be added as a new variable with the past values of $y_t$ into LSTM. The training results show the look back size of 40 is the best choice. Figure X shows the  profiles of predicted values of LSTM with solo $y_t$ as input, of LSTM with $y_t$ and $h_t$ and the true values. And the table X1 gives the MSE of the two LSTM prediction results. 


\subsection{Results analysis of statistics extraction based method}

%there are two different algorithms: rolling algorithm and non-rolling algorithm. The rolling method will keep adding the next test data into the training set and only make 1 step prediction each time;while the non-rolling method just based on the original training set and make multi-steps prediction.




































==> Experiment_bak.tex <==
\section{Performance Studies}

\note{Don't start a section with title. Write something here to introduce you work experiments etc. Say ho other people wrote.} 
\subsection{Experimental Setup}
\subsubsection{Data sets}
\rev{As typical time series data, stock prices are commonly used in data analyses. We choose three data sets on "Open Price" of different stocks in our performance studies, with each  set containing the data of one year.} \note{Any reference or links?}\note{I will do all the reference work later}  %The stock data  \rev{have} large fluctuations as well as randomness.
\rev{Stock data are typical time series in our lives. Therefore, choosing stock data for research has  good practical application value.} %The t does have a strong relationships among the current time and its past.
\del{Thus, dealing with the chaotic financial data will be a challenging but meaningful work.} The first data set is the daily open stock price for ”AMZON(AMZN)” from 01-02-2019 to 12-18-2019. \rev{The second data set is the daily open stock price for "Fidelity National Information Services(FIS)" from 01-02-2019 to 12-18-2019.}\rev{The third one is "WARMALT(WMT)" from 01-02-2019 to 12-18-2019.} We divide the data into two subsets, $88\%$ belongs to the training set and the remaining $12\%$ is used as the test set. \rev{The training set has 214 samples and test set has 28 samples. In order to further investigate the performance of our proposed methods, we  divide the test data into four subgroups: test set 1(with one week's data from day 1 to day 7);test set 2(with two weeks' data from day 1 to day 14);test set 1(with three weeks' data from day 1 to day 21);test set 1(with one weeks' data from day 1 to day 28).Day 1 here is the first sample's date in test set.}
\rev{The first data set} is represented as $y_t$ and is used as the primary example to show the performance of our methods. \note{You need to introduce all datasets, and performance metrics you use in this study.}

\subsubsection{Preparation for ARIMA-GARCH Model } Statistic models are often impacted by the stationary level of the data. We use ARIMA-GARCH model in our method 1. As a first step, we check if data are stationary.
 A time series {$x_t$} is strictly stationary if $f(x_1,...,x_n) = f(x_{1+h},...,x_{n+h})$, where $n$ and $h$ are positive integer numbers and $f(\bullet)$ denotes the function relationship. ARMA-GARCH can only deal with stationary data, while ARIMA-GARCH can \del{deal with non-stationary data by} transfer  non-stationary data into stationary ones.


In statistics, Augmented  Dickey-Fuller Test(ADF) test is the most popular method to help check if a time series is stationary, and the null hypothesis of ADF test indicates that the time series is not stationary.  The p-values obtained by the test is used to decide whether we should reject the null hypothesis, so the times series is considered to be stationary. If p-value is bigger than 0.05, we will accept the null hypothesis; otherwise, we will reject the null hypothesis. In our ADF test of data, the p-value is 0.6135,  so we accept the null hypothesis and conclude that the data set is not stationary. Then we transfer the data set $y_t$ to the difference 
form $\triangle$$y_t$. \note{If you work on the difference form. How to get the original data? Difference data have no physical meaning.}\note{Next paragraph show this process is just used to find the value of "d". We still build ARIMA-GARCH model for the original data set.} We do the ADF test for $\triangle$$y_t$  and get p-value of 0.01. As the null hypothesis is rejected, we conclude that $\triangle$$y_t$ is stationary. %\note{See how I made changes to write things more clearly.}

\subsubsection{ARIMA(p,d,q)-GARCH(P,Q) Model}
Based on the ADF test on our data, $y_t$ is not stationary, but its 1 time difference is stationary. Therefore, the parameter $d$ in \rev{the} ARIMA(p,d,q)-GARCH(P,Q) model for $y_t$ is 1. We use R Studio to build up the ARIMA-GARCH model for the data. To determine the parameters of the ARIMA(p,d,q) part, we use the "auto.arima" function in R studio, \note{Any reference?} and get ARIMA (5,1,2) for $y_t$ based on the AIC criterion. %The "auto.arima" will return the model with lowest AIC, BIC or AICc. Here we choose AIC as the criterion. 



%\rev{We further conduct} the model diagnostic test to see whether this model is suitable and the residuals of this model have no correlation. \note{how to determine suitable? What residual of the model means?}
%The correlation here refers to  linear correlation but the higher order correlations like squared correlation are not included. \note{Why only needs linear check? All these statements read random.} Ljung-Box test is a powerful tool to \rev{perform} this check. The null hypothesis of Ljung-Box test is the residuals have no auto-correlation. \note{I don't know what you want to say in this sentence. This sentence also has a wrong grammar, and not readable.} The p-values of the Ljung-Box test \note{What is the relationship between this test and ADF test?}  from lag 2 to 20 are all bigger than 0.05. We will accept the Ljung-Box test and conclude \rev{that} ARIMA(5,1,2) model is suitable. \note{It is unclear what you mean acceptable, and why it is suitable, and what you mean suitable.}

%\note{You put many buzz words without explanations, and also don't provide any reference.}

Next, the arch effect will be checked to see whether  the variance of the residuals are homogeneous. If  an arch effect exists in the model, which means the variance of the residuals are not homogeneous,  GARCH model needs to be built up to capture the data dynamics. Finally, we build up ARIMA(5,1,2)-GARCH(1,1) model for ${y_t}$ based on the AIC criterion.



\rev{As for the prediction of this model, We use the training data to build up the ARIMA(p,d,q)-GARCH(P,Q) and make prediction. Assuming the training data are ${y_1,y_2,...,y_m}$,the one step forward prediction will predict $y_{m+1}$. Next, the true value of $y_{m+1}$ will be added into ${y_1,y_2,...,y_m}$ as} ${y_1,y_2,...,y_m,y_{m+1}}$ to predict $y_{m+2}$, %which is  still based on the same ARIMA(p,d,q)-GARCH(P,Q) structure obtained in the training stage. 
\rev{The coefficients of ARIMA(p,d,q)-GARCH(P,Q) will be recomputed but the structure, i.e., $\alpha_i$,$\theta_j$,but the model structure, i.e., $(p,d,q)$ and $(P,Q)$ won't be changed.}
%\subsubsection{Proposed decomposition methods and baselines}

\subsubsection{\rev{Setting of the decomposition method}}

%\note{I am working on revising the this section now}

%\note{Are you done with the beginning part of this section?}

%\note{ what I left is the performances studies part}

 In this study, we use LSTM  as  baseline method to directly learn the data distribution and make one step forward prediction. \del{ certain number of sequence data will be took as input to predict the next. For example,} We take ${y_1,y_2,...,y_k}$ as an input and ${y_{k+1}}$ as an output to perform the training. The "Keras" with version of '2.3.1' is used to built up LSTM. "Keras" is a high-level neural networks API, written in Python, which is capable of running on top of Tensorflow. \del{LSTM or SVR.} \del{The value of $k$ is \rev{an} important parameter \rev{to learn from} the data.}\note{Do people normally learn k? If this is not predetermined, how to even perform training? } In LSTM method, \rev{given 
the input and the output,  the weights of input gates, cell states, forget gates and output gates need to be learnt }\note{What do you mean the number of units?} \del{is another parameter need to be learnt.} \note{Do people normally don't set up the number of units in advance, but learn? Then how could training be performed? Also, don't you need to learn gate parameters?} In addition, we choose " Mean squared Error" as the loss function and  $tanh$ \rev{as activation function} to do the training.  %In the SVR method, the penalty parameter C of the error term, the  $\epsilon-$insensitive loss function and the kernel function are the three key parameters need to be learnt. 

In our proposed decomposition method, we apply ARIMA-GARCH to model the stable data components to get the residual ${r_t}$ of the data. We use LSTM  as \del{two} candidate method to learn the distribution of the residual data, and have \rev{method as  ARIMA-GARCH-LSTM} \del{and have two methods ARIMA-GARCH-LSTM and ARIMA-GARCH-SVR respectively.} In the training stage, \rev{LSTM} is used to train ${r_t}$, where ${r_1,r_2,...,r_k}$ serve as the input and ${r_{k+1}}$ is the output. In the prediction stage, if we want to predict ${y_{t+1}}$, the predicted ${r_{t+1}}$ will be added to the predicted value of ${y_{t+1}}$ from ARIMA-GARCH to get the final prediction of ${y_{t+1}}$. 



\subsubsection{\rev{Setting of the method based on statistics extraction}}
\rev{The GARCH term--$h_t$, obtained from equation 8, is a statistics that can reflect the volatility of a time sequence at each time point. In our proposed statistics extraction method, the ARIMA-GARCH model will be built up for the data first, then $h_t$ can be got from this model. Next, as a new feature, $h_t$ will be put into the LSTM with $y_t$ to help capture the dynamic of $y_t$.}


%\subsubsection{Metrics}
\rev{\subsection{Metrics}} 
\note{Or any suitable name?}
We adopt four common metrics to evaluate the effectiveness of the proposed frameworks, which include  Mean Squared Error(MSE), Root Mean Squared Error (RMSE), Mean Absolute Error (MAE),and Mean Absolute Percentage Error (MAPE). \note{If you have space, you may give basic definition for each.} \rev{For all the metrics, the lower the value, the better the performance of the corresponding models.} The definitions of the four metrics are as follows:

%\note{Do you need to introduce how you get the statistics and what are the statistics? Or these statistics are varying over time as well? }
\subsection{\rev{Performance Studies}}

%\note{You need to introduce you experiment setup, metrics and datasets used that are common used for all studies at the beginning. You need to cite the dataset if it is publicly available.}

\subsubsection{Results of Decomposition Method}
%\note{This belongs of experiment setting. If it is common to all methods, move it to the beginning part.} 
We \del{first} compare the performance of different methods in making one-step forward prediction.\rev{Figure show the predictions' curves  and  Table \ref{tab1} shows the prediction results of our proposed models and the baseline models for all the four test sets.}
\del{for the first week of the data from the test set}. Compared with ARIMA-GARCH, \del{SVR} and LSTM, \del{both ARIMA-GARCH-SVR and} ARIMA-GARCH-LSTM  achieve\rev{s} better performance in all metrics.\rev{Taking results in data set 4(the whole test set) as an example, the MSE, RMSE, MAE and MAPS of the proposed model improve $38.63\%$, $21.66\%$, $27.97\%$ and $27.61\%$ compared with LSTM model and $5.43\%$, $2.76\%$, $8.64\%$ and $8.53\%$ compared with ARIMA-GARCH model, }which demonstrates the effectiveness of the decomposition method in improving the prediction accuracy. 
%\note{Why  ARIMA-GARCH-LSTM is better than ARIMA-GARCH-SVR? Explain the possible reason.}
%ARIMA-GARCH-LSTM is the best model compared with ARIMA-GARCH and LSTM. The reaso why our proposed models will outperform the baselines is we always use the suitable models to deal with the suitable data.  

\note{Does the statistic model use all data or testset data only?} \note{Answered in ARIMA-GARCH part in left column}
 %\rev{Table \ref{tab2} shows the result of the following week.} \note{Why do you show the following week? Any particular reason, or just another set of data?}
%Compared with the Table 1, 
\rev{Further, comparing the results in different test sets of Table \ref{tab1}}, the performance improvement of \del{Table \ref{tab2}} test set 1 is bigger. \rev{Figure 2 shows the predictions' curves in test set 2. This plot clearly shows the curve of ARIMA-GARCH-LSTM is the closest one to the true values' curve.}\rev{the MSE, RMSE, MAE and MAPS of the proposed model improve $66.56\%$, $42.17\%$, $50.57\%$ and $50.35\%$ compared with LSTM model and $30.97\%$, $16.92\%$, $20.80\%$ and $20.71\%$ compared with ARIMA-GARCH model.} \rev{The different performance improvement} is because that our proposed \rev{method is} built up on the base of ARIMA(p,d,q)-GARCH(P,Q) model.  When \rev{new data are} added, we just recompute the coefficients of ARIMA(5,1,2)-GARCH(1,1) model, i.e., \rev{$\alpha_i$,$\theta_j$,}but we \rev{don't} change the structure, i.e., $(p,d,q)$ and $(P,Q)$ of this model. \note{Aren't the parameters of these structures changed?} Nevertheless, as time goes by, the structure may have some changes \rev{due to the fact that financial data have more volatility. When long sequence of the new data added into the training data, the whole structure of this data may change}, so the accuracy of  ARIMA-GARCH model reduces and the residual data may have a large variation. \note{Your parameters for the statistics are not from historical data but only from recent data? Then you need to justify it and mention the finance data re volatile and you cannot use too long history data.} All these factors will affect the performances of  ARIMA-GARCH-LSTM \del{and ARIMA-GARCH-SVR} model. %But for the one step forward prediction of next one week, few data are added to ARIMA-GARCH, so the performance of ARIMA-GARCH will not be affected a lot.   \note{This is confusing. You just said for the next week, it changes a lot. Now you said it does not change a lot. Can't you be more strict in your writing?} 
Therefore, our proposed methods have better performances \rev{in all test sets especially in the first test set}

%\note{Again, you are attracting people to attack you by emphasizing show-period prediciton. People will ask what the result for long-term prediction?} Table \ref{tab3} lists the percentage improvement between different methods. \rev{Compared to  ARIMA-GARCH, the improvement of ARIMA-GARCH-SVR is larger than that of ARIMA-GARCH-LSTM, which indicates that SVR can better track the variation of residual data than LSTM.} 

%\note{I am not sure if you want to emphasize one-step prediction, if you don't study multi-step. When you said one step-forwarding of a week, it is unclear you predict a whole week or for each day you make a prediction.}


 


%And that is why the predictions for the following one week are have more improvements. 

%Figure ~\ref{LSTM38}shows the prediction results from "11/05/2018" to "01/01/2019" for ARIMA-GARCH-LSTM, ARIMA-GARCH and LSTM models. Figure ~\ref{LSTM7} shows the next one week prediction  results from "11/05/208" to "11/13/2018". 
\rev{Moreover},All the predictions in the figures shows \rev{a} first-order-lag, which means the prediction on \rev{the} day $t$ is more close to the result in \rev{the} day $t-1$. \del{To better understand the lag problem,} Taking figure ~\ref{AGL7} as an example, if we move the \rev{true} data from 1-6 to the position 2-7, you will \rev{find the results from all methods have the same trend of change.} The lag problem is a common \del{problem} in time series analysis \rev{as} the prediction results of all methods have a tendency to approach \rev{those of the} previous step.  

%The percentage improvements of our proposed methods compared with the baseline models are given in Table \ref{tab3}. From  Table \ref{tab3}, one can see LSTM and SVR both have  huge improvements when combined with ARIMA-GARCH method Although LSTM seems having worst performance compared with other models, it still has good ability to predict the tendency of the complex data. In our proposed method, we use LSTM to predict the unstable part, which 

% Please add the following required packages to your document preamble:
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
% Please add the following required packages to your document preamble:
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\footnotesize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 &  & MSE & RMSE & MAE & MAPE \\ \hline
 & AG & 156.93 & 12.53 & 10.13 & 0.57 \\ \cline{2-6} 
Test Set 1 & LSTM & 323.92 & 18.00 & 16.23 & 0.90 \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}c@{}}AG-\\ LSTM\end{tabular} & \textbf{108.32} & \textbf{10.41} & \textbf{8.02} & \textbf{0.45} \\ \hline
 & AG & 155.33 & 12.46 & 10.56 & 0.60 \\ \cline{2-6} 
Test Set 2 & LSTM & 280.57 & 16.75 & 14.38 & 0.81 \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}c@{}}AG-\\ LSTM\end{tabular} & \textbf{108.06} & \textbf{10.40} & \textbf{8.34} & \textbf{0.47} \\ \hline
\end{tabular}
\caption{\label{tab1}Metrics Analysis of Test Set 1 and Test Set 2}
\end{table}

%\caption{\label{tab1}Metrics Analysis of Test Set 1 and Test Set 2}


\begin{table}[]
\footnotesize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 &  & MSE & RMSE & MAE & MAPE \\ \hline
 & AG & 287.66 & 16.96 & 13.92 & 0.78 \\ \cline{2-6} 
Test Set 3 & LSTM & 440.38 & 20.99 & 17.34 & 0.97 \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}c@{}}AG-\\ LSTM\end{tabular} & \textbf{263.40} & \textbf{16.23} & \textbf{12.35} & \textbf{0.70} \\ \hline
 & AG & 238.25 & 15.44 & 12.39 & 0.70 \\ \cline{2-6} 
Test Set 4 & LSTM & 367.18 & 19.16 & 15.71 & 0.88 \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}c@{}}AG-\\ LSTM\end{tabular} & \textbf{225.32} & \textbf{15.01} & \textbf{11.32} & \textbf{0.64} \\ \hline
\end{tabular}
\caption{\label{tab2}Metrics Analysis of Test Set 3 and Test Set 4}
\vspace{-15pt}
\end{table}

%Metrics Analysis of Test Set 3 and Test Set 4
%\begin{table}[]
%\caption{\label{tab1}Metrics Analysis of Test Set Predictions}
%\vspace{-5pt}
%\footnotesize
%\begin{tabular}{|c|c|c|c|c|}
%\hline
% & MSE & RMSE & MAE & MAPE \\ \hline
%AG & 0.001318 & 0.036298 & 0.024794 & 2.142506 \\ \hline
%LSTM & 0.002165 & 0.046528 & 0.040433 & 3.349739 \\ \hline
%AG-LSTM & \textbf{0.001241} & \textbf{0.035234} & \textbf{0.022233} & \textbf{1.941214} \\ \hline
%SVR & 0.001501 & 0.038747 & 0.029667 & 2.510208 \\ \hline
%AG-SVR & \textbf{0.001287} & \textbf{0.035871} & \textbf{0.023604} & \textbf{2.051793} \\ \hline
%\end{tabular}
%\end{table}

%\begin{table}[]
%\caption{\label{tab2}Metrics Analysis of Following week Predictions}
%\vspace{-5pt}
%\footnotesize
%\begin{tabular}{|c|c|c|c|c|}
%\hline
% & MSE & RMSE & MAE & MAPE \\ \hline
%AG & 0.000282 & 0.016798 & 0.013751 & 1.076193 \\ \hline
%LSTM & 0.001359 & 0.036868 & 0.033778 & 2.576865 \\ \hline
%AG-LSTM & \textbf{0.000244} & \textbf{0.015636} & \textbf{0.011847} & \textbf{0.929590} \\ \hline
%SVR & 0.000273 & 0.016518 & 0.012974 & 1.007235 \\ \hline
%AG-SVR & \textbf{0.000182} & \textbf{0.013501} & \textbf{0.009888} & \textbf{0.772916} \\ \hline
%\end{tabular}
%\end{table}

%\begin{table}[]
%\caption{\label{tab3}Percentage Improvement of the Following week Predictions}
%\vspace{-10pt}
%\footnotesize
%\begin{center}

%\begin{tabular}{|c|c|c|c|c|}
%\hline
%$\%$ & MSE & RMSE & MAE & MAPE \\ \hline
%\begin{tabular}[c]{@{}c@{}}AG-LSTM \\ vs. AG\end{tabular} & 13.35 & 6.92 & 13.85 & 13.62 \\ \hline
%\begin{tabular}[c]{@{}c@{}}AG-LSTM \\ vs. LSTM\end{tabular} & 82.01 & 57.59 & 64.93 & 63.93 \\ \hline
%\begin{tabular}[c]{@{}c@{}}AG-SVR \\ vs. AG\end{tabular} & 35.40 & 19.63 & 28.09 & 28.18 \\ \hline
%\begin{tabular}[c]{@{}c@{}}AG-SVR \\ vs. SVR\end{tabular} & 33.20 & 18.27 & 23.78 & 23.26 \\ \hline
%\end{tabular}
%\end{center}
%\end{table}


\begin{figure}
  \vspace{-10pt}
  \begin{center}
\includegraphics[width=2.5 in]{images/AGL28.png}
  \end{center}
  \vspace{-10pt}
  \caption{\footnotesize Predictions of AG-LSTM and its baselines for test set 4}
\label{AGL28}
  \vspace{-10pt}
\end{figure}

\begin{figure}
  \vspace{-10pt}
  \begin{center}
\includegraphics[width=2.5 in]{images/AGL7.png}
  \end{center}
  \vspace{-10pt}
  \caption{\footnotesize Predictions of AG-LSTM and its baselines for test set 1}
\label{AGL7}
  \vspace{-10pt}
\end{figure}

\begin{figure}
  \vspace{0pt}
  \begin{center}
\includegraphics[width=2.5 in]{images/LG28.png}
  \end{center}
  \vspace{-10pt}
  \caption{\footnotesize Predictions of LSTM-GARCH and its baselines for test set 4}
\label{LG28}
  \vspace{-20pt}
\end{figure}

\begin{figure}
  \vspace{-45pt}
  \begin{center}
\includegraphics[width=2.5 in]{images/LG7.png}
  \end{center}
  \vspace{-10pt} 
  \caption{\footnotesize Predictions of AG-LSTM and its baselines for test set 1}
\label{LG7}
  \vspace{-20pt}
\end{figure}

\subsubsection{Results of \rev{Learning with Statistics Extraction}}
\rev{We compare the performance in  making  one-step  for-ward  prediction. Figure 3 shows the curve of true values and  the predictions curves of LSTM-GARCH model, ARIMA-GARCH model and LSTM model. The LSTM-GARCH model's prediction curve is the closet one to the true values. } Table 3 shows the prediction results for LSTM,ARIMA-GARCH adn LSTM-GARCH \rev{ for all the four test sets.}LSTM-GARCH is seen to be perform \note{or performing} better in all metrics. \rev{Taking the test set 4(the whole test set) as an example, The improvement of MSE, RMSE, MAE and MAPE are 
$36.87\%$,$20.55\%$,$23.91\%$,$23.55\%$ compared with LSTM model.}This demonstrates that the introduction of additional statistic feature into the learning platform has a big impact on the performance. of LSTM model.\rev{ In addition, the improvement of MSE, RMSE, MAE and MAPE are 
$2.71\%$,$1.36\%$,$3.50\%$,$3.40\%$ compared with ARIMA-GARCH model. LSTM-GARCH still has better performance than ARIMA-GARCH model.}

\begin{table}[]
\footnotesize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 &  & MSE & RMSE & MAE & MAPE \\ \hline
 & AG & 156.93 & 12.53 & 10.13 & 0.57 \\ \cline{2-6} 
Test Set 1 & LSTM & 323.92 & 18.00 & 16.23 & 0.90 \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}c@{}}LSTM-\\ GARCH\end{tabular} & \textbf{125.01} & \textbf{11.18} & \textbf{8.53} & \textbf{0.48} \\ \hline
 & AG & 155.33 & 12.46 & 10.56 & 0.60 \\ \cline{2-6} 
Test Set 2 & LSTM & 280.57 & 16.75 & 14.38 & 0.81 \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}c@{}}LSTM-\\ GARCH\end{tabular} & \textbf{149.39} & \textbf{12.22} & \textbf{10.05} & \textbf{0.57} \\ \hline
\end{tabular}
\caption{\label{tab3}Metrics Analysis of LSTM-GARCH and it's baselines for test set 1 and test set 2}
\end{table}



%\caption{\label{tab3}Metrics Analysis of LSTM-GARCH and it's baselines for test set 1 and test set 2}


\begin{table}[]
\footnotesize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 &  & MSE & RMSE & MAE & MAPE \\ \hline
 & AG & 287.66 & 16.96 & 13.92 & 0.78 \\ \cline{2-6} 
Test Set 3 & LSTM & 440.38 & 20.99 & 17.34 & 0.97 \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}c@{}}LSTM-\\ GARCH\end{tabular} & \textbf{285.41} & \textbf{16.89} & \textbf{13.70} & \textbf{0.77} \\ \hline
 & AG & 238.25 & 15.44 & 12.39 & 0.70 \\ \cline{2-6} 
Test Set 4 & LSTM & 367.18 & 19.16 & 15.71 & 0.88 \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}c@{}}LSTM-\\ GARCH\end{tabular} & \textbf{231.80} & \textbf{15.22} & \textbf{11.95} & \textbf{0.67} \\ \hline
\end{tabular}
\caption{\label{tab4}Metrics Analysis of LSTM-GARCH and it's baselines for test set 3 and test set 4}
\end{table}

%Metrics Analysis of LSTM-GARCH and it's baselines for test set 3 and test set 4



%\del{The last row of Table 4 is the percentage improvement the LSTM-GARCH model has compared with LSTM model for the whole test data.} \rev{ The improvement of RMSE is $27\%$, while the improvements of MSE, MAE and MAPE are all over $40\%$. 
\rev{Further, comparing the results in different test sets of table 3, the performance  of test set 1 is has the biggest improvement.}The MSE, RMSE, MAE and MAPE in our proposed method has improved $61.41\%$,$37.88\%$,$47.48\%$,$47.29\%$ compared with LSTM model and $20.34\%$,$10.77\%$,$15.85\%$,$15.82\%$ compared with ARIMA-GARCH. The reason is similar to that in the last part. When a long sequence of the new data added into the training data, the whole structure of this data may change, so the accuracy of  ARIMA-GARCH model reduces and the GARCH term($h_t$) obtained by ARIMA-GARCH model may have a large variation.
%This demonstrates that the introduction of additional statistic feature into the learning platform has a big impact on the performance. \del{}LSTM model.}
\note{I will not put baseline results again in table 5 due to the page limits}


In Table 5, we further compare the performance between the methods 1 and 2. \del{in preference to the base lines ARIMA-GARCH and LSTM.} ARIMA-GARCH-LSTM \rev{not only} outperforms the baselines ARIMA-GARCH and LSTM in all metrics \rev{but also} is superior to our proposed  LSTM-GARCH model. The reason is that the decomposition method  extracts data information more sufficiently while LSTM-GARCH just utilizes the GARCH term to help improve the LSTM performance. However, the second method is more concise and easy to use while the first method need more pre-work to do. 


%\rev{Compared with the decomposition-based method, the method of learning with statistic extraction has more freedom and can better track the practice data.} Finally, we conclude that the extraction method not only  improves the performance of LSTM but have better sustainability compared with the decomposition method. \note{Why?You cannot simply claim.}

%We can conclude our statistics extraction method did improve a lot. 



%\begin{table}[]
%\caption{\label{tab4}Metrics Analysis of Test Set Predictions}
%\vspace{-5pt}
%\footnotesize
%\begin{tabular}{|c|c|c|c|c|}
%\hline
 %& MSE & RMSE & MAE & MAPE \\ \hline
%LSTM & 0.002165 & 0.046528 & 0.040433 & 3.349739 \\ \hline
%\begin{tabular}[c]{@{}c@{}}LSTM-\\ GARCH\end{tabular} & 0.001142 & 0.033791 & 0.021945 & 1.897688 \\ \hline
%\begin{tabular}[c]{@{}c@{}}LSTM-\\ GARCH\\ vs.LSTM($\%$)\end{tabular} & 47.26 & 27.37 & 45.73 & 43.35 \\ \hline
%\end{tabular}
%\vspace{-5pt}
%\end{table}


%\begin{table}[]
%\caption{\label{tab5}Metrics Comparisons among extraction, decomposition and baseline methods }
%\vspace{-5pt}
%\footnotesize
%\begin{tabular}{|c|c|c|c|c|}
%\hline
% & MSE & RMSE & MAE & MAPE \\ \hline
%AG & 0.001318 & 0.036298 & 0.024794 & 2.142506 \\ \hline
%LSTM & 0.002165 & 0.046528 & 0.040433 & 3.349739 \\ \hline
%AG-LSTM & 0.001241 & 0.035234 & 0.022233 & 1.941214 \\ \hline
%\begin{tabular}[c]{@{}c@{}}LSGM\\ -GARCH\end{tabular} & \textbf{0.001142} & \textbf{0.033791} & \textbf{0.021945} & \textbf{1.897688} \\ \hline
%\end{tabular}
%\vspace{-10pt}
%\end{table}


%\begin{figure}
 % \vspace{5pt}
 % \begin{center}
%\includegraphics[width=2.5 in]{images/LG38.png}
 % \end{center}
 % \vspace{-10pt}
 % \caption{\footnotesize Open Price Predictions}
%\label{LG38}
 % \vspace{-10pt}
%\end{figure}




\subsubsection{Robust Analysis}
\rev{We use two more data sets to test the superiority of our proposed. The first one is the stock open Price of "Fidelity National Information Services(FIS)" from 01-02-2019 to 12-18-2019 and the second one is the stock open Price of "Walmart(WMT)" from 01-02-2019 to 12-18-2019.} The metrics analysis of method 1, method 2 and their baselines for all the test sets are put into one table. Table 6 and 7 shows the result of "FIS" and "WMT",respectively.  One can see our proposed models have best performance compared with the baselines for all the test sets. Therefore, we conclude that both the decomposition method and the statistics extraction method 
are exceptional and deserve more attention.

\subsubsection{Conclusion}







%We use two more data sets \note{Did you introduce this somewhere?} to test the superiority of our proposed \rev{methods. Tables} 6 and 7 show the prediction results \rev{for a  longer time period and one week respectively. Both our methods perform better than the baseline models.} \del{both in Table 6 and Table 7.} The results in Table 7 have much more \rev{performance} improvement compared with that in Table 6. The reason is similar to data set 1.  \note{You didn't explain this earlier, between a long data set and short one. I didn't put whole data set to avoid problem.} \note{Also, why you didn't show the performance of extraction-based method?} 

\begin{table}[]
\footnotesize
\begin{tabular}{|l|l|l|l|l|l|}
\hline
 &  & MSE & RMSE & MAE & MAPE \\ \hline
{Test Set 1} & \begin{tabular}[c]{@{}l@{}}AG-\\ LSTM\end{tabular} & 108.32 & 10.41 & 8.02 & 0.45 \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & \begin{tabular}[c]{@{}l@{}}LSTM-\\ GARCH\end{tabular} & 125.01 & 11.18 & 8.53 & 0.48 \\ \hline
{Test Set 2} & \begin{tabular}[c]{@{}l@{}}AG-\\ LSTM\end{tabular} & 108.06 & 10.40 & 8.34 & 0.47 \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}l@{}}LSTM-\\ GARCH\end{tabular} & 149.39 & 12.22 & 10.05 & 0.57 \\ \hline
{Test Set 3} & \begin{tabular}[c]{@{}l@{}}AG-\\ LSTM\end{tabular} & 263.40 & 16.23 & 12.35 & 0.70 \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}l@{}}LSTM-\\ GARCH\end{tabular} & 285.41 & 16.89 & 13.70 & 0.77 \\ \hline
{Test Set 4} & \begin{tabular}[c]{@{}l@{}}AG-\\ LSTM\end{tabular} & 225.32 & 15.01 & 11.32 & 0.64 \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}l@{}}LSTM-\\ GARCH\end{tabular} & 231.80 & 15.22 & 11.95 & 0.67 \\ \hline
\end{tabular}
\caption{\label{tab5} Metrics comparisons of AG-LSTM and LSTM-GARCH for all test sets.}
\end{table}




==> Introduction.tex <==
\section{Introduction}

In recent years, we are seeing a rapid growth of data from the increasing deployments of sensors and sources of various types. The availability of massive data calls for new and more advanced schemes to analyze the data, and apply the knowledge to  enable more intelligent and powerful applications.  Data-based (model-less) applications attempt to extract information directly from the data without preprocessing through complex models. Machine learning systems are becoming increasingly employed in complex high-stakes settings such as medicine (e.g. radiology, drug development), financial technology (e.g. stock price prediction, digital financial advisor), and even in law (e.g. case summarization, litigation prediction). Despite this increased utilization, there is still a lack of sufficient techniques available to be able to explain and interpret the decisions of these deep learning algorithms.

The convergence of data and model has been reflected from at least two aspects. First, massive data have transformed the way how system states can be estimated and predicted, which is essential for reliable system operations and decision making. Second, data also provide a venue to critically examine and refine traditional “model-based” methods for many applications. These have led to the “data-driven” methods that have greatly empowered the applications. However, a subtle issue is how to properly integrate data-driven methods with existing knowledge or models. After all, many application field have been extensively studied for the last almost a century, and has well-established theories and models. Data, big or small, can better reflect the knowledge or help discover new knowledge, but are not expected to fundamentally change the established knowledge. Therefore,maximizing the potential of data-driven methods while at the same time respecting basic theories and knowledge to enable new and powerful applications is currently a grand challenge.

The introduction of new information may be helpful to  improve the performance of both the model-based and data-based learning. However, a more valuable research is how to integrate models without introducing new information to improve the performance of the model. To achieve this goal, in this paper, we propose three methods, which give 3 directions to integrate both model based and data based learning to produce "1+1 $>$ 2" effect. The first one presents a  way of decomposing the data into different parts, such as linear stable part, nonlinear stable part  and unstable part. The mathematical models will model both the linear and nonlinear stable parts while the machine learning method will handle the unstable part. The mathematical models can account for most of data; as for the unstable part, machine learning method will take effect. The merit of this method is that it improves the predictive ability of the model without reducing model interpretation, and has better performance than the single used mathematical models and machine learning methods. The second method starts from a completely different perspective from the first method. Not based on the decomposition of the data, but relying on the extraction of statistics come from mathematical models. It still uses mathematical statistics models to model first, then extracts valuable statistics information, and finally feeds the extracted statistics as new features into the machine learning learner for training. The contribution here is not the method of adding new features into the machine learning learner but the thought of how to incarcerate model based and data based learning and the way to generate and extract new features. Different from the  ways of adding new features by introducing new information to help boost the learning ability, our method acquires new features without any new information. Take time series data as an example, after the ARIMA-GARCH model established, the GARCH term, that is conditional variance, is noticed by us due to the Time-varying characteristics. Then we propose to utilize the GARCH term as a new feature to be fed into the machine learner to improve model performance. In the third method, we consider to incorporate both the first two methods to better improve the performance of the learners. On the basis of  decomposition method, method 2 is applied to model and make prediction for the unstable part.

==> M+D.tex <==
\section{\rev{Modeling Time Series Data with Model-driven and Data-driven Components}}
\vspace{-0.10in}
\note{ Don't put method, scheme, etc in the title. people knows it is a method, or a scheme. Don't put novel, which only gives people bad impression. You need to convince people it is novel with your description, but not to claim it is novel.  It triggers the anger.}



\note{You need to pay attention how English sentences are written formally from paper reading. Your writing is too oral and informal. Also comparing my writing and your previous writing to see the difference. See why I reorganize your writing each time to make the logic more natural.}

\rev{In order to more accurately model the time series data while reducing the complexity and increasing  interpretability, we explore the use of both  model-driven  and data-driven approaches. Generally, statistical models can well represent stable data with slow variations, but are not good at tracking dynamic data with fast changes. Purely relying on neural network to track data, however, may suffer from long training time and low interpretability. We first introduce a decomposition-based method to exploit both types of technique.  We decompose each data item into multiple parts.  For each part, we choose a specific model that can best represent the data based on the features of the part.}


\note{You are not decomposing a data set to multiple parts, but each data item to multiple parts, right?} \note{Yes! Not  decomposing a data set but for each data item to multiple parts.}
%\rev{In order to more accurately model the data while reducing the complexity and increasing  interpret-ability, fully explore the information of the data itself and enhance the interpret-ability of the model, some model-driven + data-driven approaches can be considered. In this section, assuming we just have one time series data, our major goal is to boost the current model-driven or data-driven methods just based on the single time series data we have without introducing any other information. Primarily we have two different directions to achieve our goal: The first one is to introduce the data decomposing method. \sout{According to the learning abilities  of statistical time series model and machine learning model}, we decompose the data set into different parts. For each part, we use the specific model with the best learning capacity to train and model. The motivation here is we believe that statistical methods and machine learning methods both have their own advantages and limitations. After the data is decomposed, choosing the optimal modeling method according to the characteristics of different parts can make full use of the advantages of different learners, improve the learning ability of the entire time series data, and make the prediction more accurate. }


\rev{Statistic models are limited if the the parameters associated with the models are pre-determined. Neural networks are known to be able to more flexibly model the data without any assumption on data format. 
Without any knowledge on the data, however, it may take a long time for the training process to converge, and it is hard to explain and control the network learnt. If the statistics of the data is known, it will help speed up the training process and allow for better understanding of the data characteristics. As a second method,  we propose to extract the statistics of data and incorporate them into the pure neural-network based models to improve the learning capability. As a third method, we will design a mixed model that can concurrently exploit decomposition-based method and extraction-based method.}  

\note{This paragraph is somewhat different from what I want to express. The training time of the learning part of the first method is indeed reduced, but the training time of the second method does not decrease but will increase slightly, because it adds new features to the training. Time must be increased. So what I want to emphasize here is that after new features are added, the model's prediction accuracy will increase and the prediction ability will increase.}



%Another direction is to use statistical models to mine new valuable information or statistics to improve the learning ability of machine learning models. The usual data-driven supervised learning method mainly lies in learning the mapping relationship between input variables and output variables. While Model-based statistical methods are very concerned about the generation of certain statistics, and use different statistics to measure the distribution of the population or the sample and certain conditions of the sample itself. For example, statistical researchers will use average to assess overall quality, variance to measure fluctuations in things, or mode to judge mainstream opinions, and so on. Therefore, we want to use the statistical model to find valuable statistics first then feed these statistics into the data-driven learner to enhance the learning ability.This is our motivation of second direction. }

%\rev{In this section, section 3.1 is the method of first direction, section 3.2 is the method of second direction and section 3.3 is a boosting method based on the two directions. The performance of different methods will be shown on Section 4.}


\subsection{\rev{Modeling time series data with decomposition}}
\vspace{-0.10in}

Time series data can be divided into \rev{a} stable part and \rev{an} unstable part. \note{before a single noun, it needs to put article words a, an or the.} Generally, the stable part can be more easily modeled, while it is often hard to  accurately model the unstable part. Further, the stable part can be categorized  into two types, linear stable  and nonlinear stable. From the model features we introduce earlier, we could choose to model the linear stable part of the data with ARIMA and the nonlinear stable part with GARCH. In order to capture all possible features in practical data, we can represent the data with  ARIMA-GARCH and LSTM together, so both stable part and and unstable part of the data can be tracked. If we include the parameters into the model representation, this data can be represented with $ARIMA(p,d,q)-GARCH(P,Q)-LSTM$.  It is not difficult to see that this complete data representation can reduce to $ARIMA(p,d,q)-LSTM$ when there are only linear stable part and unstable part in the time series, that is ($P=0,Q=0$). The complete ARIMA-GARCH-LSTM model  will reduce to the GARCH($P,Q$)-LSTM model if there is no linear stable part in the time series, that is ($p=0,q=0$). Next we we introduce the detailed formats of these three representations. 

%The stable part refers to that can be modeled by the mathematical model like ARIMA and GARCH models; while the unstable part is that can't be modeled by those mathematical model. Further, the stable part can be divided into linear stable part and nonlinear stable part. Linear stable part is that can be explained by ARIMA model while the nonlinear stable part is that can be explained by GARCH model. Genrally, a hybrid ARIMA-GARCH and LSTM method can be used to model the  time series. However, ARIMA(p,d,q)-GARCH(P,Q)-LSTM model will reduce to ARIMA(p,d,q)-LSTM when there are only linear stable part and unstable part in the time series, that is (P=0,Q=0); and ARIMA-GARCH-LSTM model will reduce to GARCH(P,Q)-LSTM model if there is no linear stable part in the time series, that is (p=0,q=0).

\paragraph{Complete data representation with ARIMA-GARCH-LSTM}
\vspace{-0.10in}
As a general format, a time series $y_t$ can be represented as:
\begin{equation}
     y_t = S_t + N_t = LS_t + NS_t + N_t
\end{equation}
where $S_t$ is the  stable part, $N_t$ is the unstable part, $LS_t$ is the linear stable part and $NS_t$ is the nonlinear stable part.  $S_t$ can be modeled by ARIMA-GARCH and $N_t$ can be learnt through $LSTM$. In this case, $y_t$ can be expressed more completely as:
\begin{equation}
\begin{cases}
    y_t = \mu_0  + u_t + \widehat{LSTM} \\
    u_t = \sum_{i=1}^{p} {\alpha_i{u_{t-i}}} + e_t+ \sum_{j=1}^{q} {\theta_j{e_{t-j}}}\\
    e_t = z_t{\sqrt{h_t}}, \quad  z_t\sim N(0,1)\\
    h_t = w+\sum_{j=1}^{P}{\lambda_j{e_{t-j}^2}}+\sum_{i=1}^{Q}{\beta_i{h_{t-i}^2}}
\end{cases}
\end{equation}
where $y_t$ is a stationary time series, and $\mu_0$ is a constant. \rev{The stable part $u_t$ follows the $ARIMA-GARCH$ model and the unstable part $\widehat{LSTM}$ is learnt through $LSTM$. The random error $e_t$ is a function of $z_t$ which follows the normal distribution,  and $h_t$ is the GARCH term  (i.e. conditional variance).} $\alpha_i$, $\theta_j$, $\beta_i$ and $\lambda_j$ are the weights. 

                    
\paragraph{ARIMA-LSTM}
\vspace{-0.10in}
If a time series just includes linear stable part and unstable part, the time series can be represented as:
\begin{equation}
     y_t = LS_t +  N_t
\end{equation}
where $LS_t$ can be modeled by ARIMA model. The equation above can be expressed as:
\begin{equation}
\begin{cases}
    y_t = \mu_0 + u_t + \widehat{LSTM} \\
    u_t = \sum_{i=1}^{p} {\alpha_i{u_{t-i}}} + e_t+ \sum_{j=1}^{q} {\theta_j{e_{t-j}}} \\
    e_t\sim N(0,1) \\
\end{cases}
\end{equation}

\paragraph{GARCH-LSTM}
\vspace{-0.10in}
If a time series just includes nonlinear stable part and unstable part, the time series can be represented as:
\begin{equation}
     y_t = NS_t +  N_t
\end{equation}
where $NS_t$ can be modeled by GARCH model. The equation above can be expressed as:
\begin{equation}
    \begin{cases}
      y_t = \mu_0 + u_t + \widehat{LSTM}\\
      u_t = z_t{\sqrt{h_t}}\quad z_t\sim N(0,1)\\
      h_t = w+\sum_{j=1}^{P} {\lambda_j{u_{t-j}^2}}+\sum_{i=1}^{Q}{\beta_i{h_{t-i}^2}}
    \end{cases}
\end{equation}
\subsection{\rev{Sequential neural network with statistics extraction}}
\note{I will combine the two method and reorganize this section later}
 \rev{Good statistics values of a time series can help to better understand and capture the change of data. The average, median, mode and quantile can reflect the distribution of a data set and are used the most.} 
 %However, in time series, if one wants to use some statistics to help us model and predict, it is difficult to get help from these commonly used statistics. An important reason is that they all have only one value.
 \note{We cannot say these statistics do not have any help. Conventional statistics based method just calculate these values based on existing data and use these values in the model for the future data, right?}
 \rev{However, if these statistics are only drawn from existing data and set to fixed values, they can not well reflect the time varying features of time series data. If the statistics themselves can be modeled as time series,  they may be fed as additional input variables to help better train the sequential neural network.}
 %But if there exits a statistics that changes over time, in another word, if there is a statistics as time series data, then this kind of statistics can be fed as another input variable into the sequential neural network for training. 
 
 \rev{Apart from variables commonly used as inputs to the sequential neural network, we add in the statistics extracted from the data series as additional inputs. The GARCH term $h_t$ is a good candidate to choose. As a conditional variance, it can reflect the volatility of the sequence at different time and is essential for describing and predicting the changes of sequence. To explain our design principles, we use LSTM as an example neural network and the GARCH term $h_t$ as the example statistics. We propose two methods to incorporate the statistics into the sequential neural networks. } 
 %a conditional variance that can be  attracts our attention. 


 \rev{In method I, we use the past values of both $y_t$ and $h_t$ to train LSTM and predict the future values of $y_t$.  That is, besides past values of $y_t$ (i.e., ${y_{t}, y_{t-2},...,y_{t-k1}}$), we add past values of the GARCH term $h_t$ (i.e., ${h_{t-1}, h_{t-2},...,h_{t-k2}}$) as another input:} \note{For prediction, you may start from $y_{t+1}$}
 
% \paragraph{Method I of Multi-variables LSTM based on statistics extraction}
% \rev{Apart from the variable of time series data in the past, the GARCH term $h_t$ will be another variable to train the LSTM. In method I, past values of $y_t$ are the first input and the past values of $h_t$ will be the second input. Specifically, ${y_{t}, y_{t-2},...,y_{t-k1}}$ is the first input and ${h_{t-1}, h_{t-2},...,h_{t-k2}}$ is the second input. Method I is designed by the common sense, where we use both the past information of $y_t$ and $h_t$ to train the LSTM and predict $y_t$ in the future. The equation can be expressed as below:}
 \begin{equation}
    {y_{t}} = LSTM(y_{t-1},y_{t-2},...,y_{t-k1};h_{t-1},h_{t-2},...h_{t-k2}) + \varepsilon_t
\end{equation}
Where $\varepsilon_t$ is the random error. For the convenience of expression, we call the model above as LSTM-GARCH-I model. \note{On the left side of the above equation, will write the expression in sequential order, $y_{t}, y_{t+1}$? In the second method, you use sequential order. These two are not consistent. } 


\note{You are not using only using the current, but also future states?}

 \rev{In method II, besides past values of $y_t$ and $h_t$, we will also add the future values of $h_t$ to train the sequential neural network. As a statistic variable, $h_t$ reflects the fluctuation of $y_t$, but is also more stable thus can be better predicted than the raw data.
 %a current to current mapping between $h_t$ and $y_t$ will better capture the current data states. 
 In this case, to predict ${y_{t+k},y_{t+k-1},...,y_{t}}$,} we will not only use ${y_{t-1},y_{t-2},...,y_{t-k1}}$ and ${h_{t-1},h_{t-2},...h_{t-k2}}$, but also ${h_{t+k},h_{t+k-1},...,h_{t}}$. \rev{Although this design is easy to realize in the training phase, if multi-step prediction is needed,  we don't have the future values of ${h_{t+k},h_{t+k-1},...,h_{t}}$ in the testing phase and practical applications. To address the issue, we apply another LSTM to predict the future values of $h_t$ based on past $h_t$ values.} 
 %we train another multi-steps single-variable LSTM to  predict $h_t$ in the future. Therefore, in method II, we have trained two LSTM. The first one is trained to predict $h_t$; while the second one utilizes  the past values of  $y_t$ and the past to current values of $h_t$ as variables to train to predict $y_t$.  
 The algorithm of method II is shown below and the structure is shown in Fig. 
 
 
 \note{Normally, people use left side as past, right side as future. Your notations seem to be not used commonly.} \rev{In time series expression, people more likely to express the data from t-1 to t-n}

 
% \paragraph{Method II of Multi-variables LSTM based on statistics extraction}
% \rev{In the Method I above, the past information both of $y_t$ and $h_t$ are used to predict the future $y_t$. But in method II, we want to add the present values of $h_t$ into the past $h_t$ to train our model. The reason to do so is that $h_t$ itself reflects the  fluctuation in current time of $y_t$. A current to current mapping between $h_t$ and $y_t$ will be a more logical relationship. For example, to predict ${y_{t+k},y_{t+k-1},...,y_{t}}$, we use not only  ${y_{t-1},y_{t-2},...,y_{t-k1}}$ and ${h_{t-1},h_{t-2},...h_{t-k2}}$, but ${h_{t+k},h_{t+k-1},...,h_{t}}$. In the training phase, this design is easy to implement but in the testing phase, we don't have the future values of ${h_{t+k},h_{t+k-1},...,h_{t}}$ because we assume we just have the information before t. \sout{However, to predict the future in test stage, the future values of $h_t$ are needed but we have no information of future $h_t$.} In order to solve this problem, we train another multi-steps single-variable LSTM to  predict $h_t$ in the future. Therefore, in method II, we have trained two LSTM. The first one is trained to predict $h_t$; while the second one utilizes  the past values of  $y_t$ and the past to current values of $h_t$ as variables to train to predict $y_t$.  The algorithm of method II is shown below and the structure is shwon in Fig. }
 
 
 
 
 
 
% The mathematical expression of method II is as follows:
 \begin{equation}
    {y_t} = LSTM(y_{t-1},y_{t-2},...,y_{t-k1};h_t,h_{t-1},h_{t-2},...h_{t-k2}) + \varepsilon_t
\end{equation}
 
 
 
 \rev{We call this model as LSTM-GARCH-II.}
 

\subsection{Hybrid  time series model \rev{exploiting both  data decomposition and statistic feature extraction}}

\rev{With data decomposition,  ARIMA-GARCH is applied to model the stable part of the data, and LSTM is used to track the unstable part of the data. In the method exploiting statistic feature extraction, LSTM-GARCH takes the statistic-based time series $h_t$ as an additional input to predict $y_t$. To take full advantage of both types of method, we introduce a hybrid  model  Hybrid-LSTM-GARCH to exploit the use of both.   In this model,  a time series $y_t$ is first divided into a stable part $S_t$ and an unstable part $N_t$. Then $S_t$ is modeled by ARIMA-GARCH and  $N_t$ is modeled by LSTM-GARCH. Rather than predicting $y_t$ directly, the statistics $h_t$ is applied with LSTM to predict  $N_t$. The hybrid model is \rev{briefly} represented as}

%\rev{Hybrid  model here takes advantage of both the decomposing and statics extracting method. In section 3.2, the LSTM-GARCH method utilizes the new statistics $h_t$ to help predict $y_t$; and in section 3.1, for the complete version of model, after decomposing the data, ARIMA-GARCH is used to deal with stable part and LSTM is used to deal with unstable part. After carefully thinking about the two methods above, we found a new method that can take full advantage of the  two methods. Take the LSTM-GARCH-I model in section 3.2 for example. First of all, still dividing the time series $y_t$ into stable part $S_t$ and unstable part $N_t$. $S_t$ is molded by ARIMA-GARCH first; then the $N_t$ (not $y_t$) are modeled by LSTM-GARCH.That is, we use the new statistics $h_t$ to help predict  $N_t$ instead of $y_t$. We call this model as Hybrid-LSTM-GARCH model, which is represented as follosw:}

\begin{equation}
    y_t = S_t + N_t
\end{equation}
\begin{equation}
    N_t = LSTM(N_{t-1},N_{t-2},...,N_{t-k1};h_{t-1},h_{t-2},...,h_{t-k2})+\varepsilon_t
\end{equation}

Where $\varepsilon_t$ is the random error.
\note{Why here you only predict one step, while in the previous section you predict multiple steps? The paper does not have consistent notations everywhere.}



%\subsection{\sout{\rev{Sequential neural network based on statistical statistics feature extraction II}}}
%\sout{Based on method , a hybrid LSTM-GARCH model will be builded up to predict $y_t$. The difference between method IV and method II is method IV will take the current value of $h_t$ into consideration to predict $y_t$,} \note{Why?} that is,
%\begin{equation}
    %y_t = LSTM(y_{t-1},y_{t-2},...,y_{t-n};h_t,h_{t-1},h_{t-2},...h_{t-n}) + \varepsilon_t
%\end{equation}
%\sout{For the multiple steps prediction, method IV can be expressed as:}
%\begin{equation}
    %{y_t,y_{t+1},...,y_{t+m}} = LSTM(y_{t-1},y_{t-2},...,y_{t-n};h_{t+m},...,h_t,h_{t-1},h_{t-2},...h_{t-n}) + \varepsilon_t
%\end{equation}

%\sout{Take one step prediction for example, GARCH values $h_t$ is a single time series like $y_t$. ARIMA-GARCH model was built up first to $y_t$; then make prediction for $h_t$ by LSTM model. Next, the current GARCH value $h_t$ was added into LSTM-GARCH to predict $y_t$, which is shown in (23).} \note{At the beginning of this section you need to introduce problem and motivation and design consideration.}

==> M+D_bak.tex <==
\section{Model-driven+Data-driven Learning}
\vspace{-0.10in}
In order to better model the data, fully explore the information of the data itself and enhance the interpret-ability of the model, some model-driven + data-driven approaches can be considered.
\subsection{Hybrid model-driven+data-driven methods I}
\vspace{-0.10in}
For a time series, one can divide into stable part and unstable part. The stable part refers to that can be modeled by the mathematical model like ARIMA and GARCH models; while the unstable part is that can't be modeled by those mathematical model. Further, the stable part can be divided into linear stable part and nonlinear stable part. Linear stable part is that can be explained by ARIMA model while the nonlinear stable part is that can be explained by GARCH model. Genrally, a hybrid ARIMA-GARCH and LSTM method can be used to model the  time series. However, ARIMA(p,d,q)-GARCH(P,Q)-LSTM model will reduce to ARIMA(p,d,q)-LSTM when there are only linear stable part and unstable part in the time series, that is (P=0,Q=0); and ARIMA-GARCH-LSTM model will reduce to GARCH(P,Q)-LSTM model if there is no linear stable part in the time series, that is (p=0,q=0).

\subsubsection{ARIMA-GARCH-LSTM}
\vspace{-0.10in}
A time series $y_t$ can be represented as:
\begin{equation}
     y_t = S_t + N_t = LS_t + NS_t + N_t
\end{equation}
where $S_t$ is the  stable part, $N_t$ is the unstable part, $LS_t$ is the linear stable part and $NS_t$ is the nonlinear stable part.  $S_t$ can be modeled by ARIMA-GARCH and $N_t$ can be modeled by $LSTM$; then $y_t$ can be expressed more formally as:
\begin{equation}
\begin{cases}
    y_t = \mu_0 + \widehat{LSTM} + u_t\\
    u_t = \sum_{i=1}^{p} {\alpha_i{u_{t-i}}} + e_t+ \sum_{j=1}^{q} {\theta_j{e_{t-j}}}\\
    e_t = z_t{\sqrt{h_t}} \quad  z_t\sim N(0,1)\\
    h_t = w+\sum_{j=1}^{P}{\lambda_j{e_{t-j}^2}}+\sum_{i=1}^{Q}{\beta_i{h_{t-i}^2}}
\end{cases}
\end{equation}
where $\mu_0$ is a constant and $\widehat{LSTM}$ represents the unstable part modeled by $LSTM$ method. 
                    
\subsubsection{ARIMA-LSTM}
\vspace{-0.10in}
If a time series just includes linear stable part and unstable part, the time series can be represented as:
\begin{equation}
     y_t = LS_t +  N_t
\end{equation}
where $LS_t$ can be modeled by ARIMA model. The equation above can be expressed as:
\begin{equation}
\begin{cases}
    y_t = \mu_0 + \widehat{LSTM} + u_t\\
    u_t = \sum_{i=1}^{p} {\alpha_i{u_{t-i}}} + e_t+ \sum_{j=1}^{q} {\theta_j{e_{t-j}}}\\
\end{cases}
\end{equation}
\subsubsection{GARCH-LSTM}
\vspace{-0.10in}
If a time series just includes nonlinear stable part and unstable part, the time series can be represented as:
\begin{equation}
     y_t = NS_t +  N_t
\end{equation}
where $NS_t$ can be modeled by GARCH model. The equation above can be expressed as:
\begin{equation}
    \begin{cases}
      y_t = \mu_0 +\widehat{LSTM}+ u_t \\
      u_t = z_t{\sqrt{h_t}}\quad z_t\sim N(0,1)\\
      h_t = w+\sum_{j=1}^{P} {\lambda_j{u_{t-j}^2}}+\sum_{i=1}^{Q}{\beta_i{h_{t-i}^2}}
    \end{cases}
\end{equation}
\subsection{Hybrid model-driven+data-driven method II: LSTM-GARCH}
 GARCH values $h_t$ estimated by ARIMA-GARCH model is an important statistics. $h_t$ reflects the volatility of the sequence at different times and is essential for describing and predicting sequence changes. In the hybrid LSTM-GARCH model, $h_t$ was added into the input of LSTM model, then using LSTM method to train and make prediction, which can be expressed as below:
\begin{equation}
                                                        y_t = LSTM(y_{t-1},y_{t-2},...,y_{t-n};h_{t-1},h_{t-2},...h_{t-n}) + e_t
\end{equation}
The model above is called as Hybrid LSTM-GARCH model.
\subsection{Hybrid model-driven+data-driven method III: Residual LSTM-GARCH}
Residual LSTM-GARCH model seems like the combination of Hybrid model-driven+data-driven method I and II. ARIMA-GARCH-LSTM model and LSTM-GARCH model. Still dividing the time series $y_t$ into stable part $S_t$ and unstalbe part $N_t$. $S_t$ is molded by ARIMA-GARCH first; then the residuals(not $y_t$) are modeled by LSTM-GARCH. The Residual LSTM-GARCH can be represented as follows:
\begin{equation}
    y_t = S_t + N_t
\end{equation}
\begin{equation}
    N_t = LSTM(N_{t-1},N_{t-2},...,N_{t-n};h_{t-1},h_{t-2},...,h_{t-n})+e_t
\end{equation}
\subsection{Hybrid model-driven+data-driven method IV: xxxx}
Based on method II, a hybrid LSTM-GARCH model will be builded up to predict $y_t$. The difference between method IV and method II is method IV will take the current value of $h_t$ into consideration to predict $y_t$,that is,
\begin{equation}
    y_t = LSTM(y_{t-1},y_{t-2},...,y_{t-n};h_t,h_{t-1},h_{t-2},...h_{t-n}) + e_t
\end{equation}
For the multiple steps prediction, method IV can be expressed as:
\begin{equation}
    {y_t,y_{t+1},...,y_{t+m}} = LSTM(y_{t-1},y_{t-2},...,y_{t-n};h_{t+m},...,h_t,h_{t-1},h_{t-2},...h_{t-n}) + e_t
\end{equation}
Take one step prediction for example, GARCH values $h_t$ is a single time series like $y_t$. ARIMA-GARCH model was built up first to $y_t$; then make prediction for $h_t$ by LSTM model. Next, the current GARCH value $h_t$ was added into LSTM-GARCH to predict $y_t$, which is shown in (23). 

==> Model.tex <==
\section{Preliminaries}
Various types of statistical models have been developed in the literature to represent the time series data for different applications. In recent years, increasing attentions are drawn to apply neural networks and \rev{machine} learning to represent complex data distributions. Before presenting our proposed methods, we review some basic statistical models commonly used to model financial data, and basic neural network structure \rev{and machine learning technique} used to represent time series data. 

\subsection{Statistic Models}
To represent the time series data, statistic models have been developed in the literature. Compared to methods using the neural networks, they can better explain the relationship between data and reveal the mechanism of change among data. In addition, model-base methods have good analytical properties, and can better calculate and theoretically prove the existence and convergence of errors. Taking daily financial stock data as an example, the data constantly change over time. Parameters, such as daily open price, close price, maximum price and minimum price, always change but have some relationships with the data of previous days. For example, the daily close price in day $t$ may be related with those in day $t-1, t-2…t-10$. Generally, the influences from closer days are bigger.  The task for model-based methods is to find and capture the strong relationship among the data in day $t$ and the data in previous days. A few models are commonly used to represent financial data. 

\paragraph{ARMA Model}

ARMA (Auto-Regressive Moving Average) is a general model used to forecast a stationary time series. ARMA ($p,q$) is a combination of Auto-Regressive(AR($p$)) process and Moving Average(MA($q$)) process. AR($p$) is generally written as 
\begin{equation}
				y_t = \mu + \alpha_1{y_{t-1}}+\alpha_2{y_{t-2}}+...+\alpha_p{y_{t-p}}+e_t,
\end{equation}
where $y_t$ is a stationary time series, $\mu$ is a constant, $\alpha_1,\alpha_2,...\alpha_p$ are the auto-correlation coefficients at lags 1,2…$p$. \rev{The residual $e_t$ is often assumed to be Gaussian white noise with the mean zero and the variance $\sigma_t$}.  To improve \rev{the accuracy of time series prediction, MA($q$) forecasts} the lagged values of the errors:
\begin{equation}
	y_t = \mu + e_t+\theta_1{e_{t-1}}+\theta_2{e_{t-2}}+....+\theta_q{e_{t-q}},
\end{equation}
where $\mu$ is the expectation of $y_t$ (usually assumed equal to zero), $\theta$ terms are the weights for prior stochastic term in time series. $e_t$ is often assumed to follow Gaussian white noises with mean zero and variance $\sigma_t$. 
%where $p$ is number of lagged observations for the auto-regression model, which uses the dependencies between an observation and the lagged observations; $q$ is number of lagged forecast residual errors for the moving average model, which uses the dependency between observations and the lagged forecast errors. 
Integrating AR($p$) and MA($q$), ARMA($p$,$q$) model is expressed as
\begin{equation}
   y_t = \mu + \sum_{i=1}^{p} {\alpha_i{y_{t-i}}} + e_t+ \sum_{j=1}^{q} {\theta_j{e_{t-j}}}.
\end{equation}

\paragraph{ARIMA Model}

 To model the non-stationary time series data,  Auto-Regressive Integrated Moving Average(ARIMA) is used to generalize ARMA model with ARMA($p$,$d$,$q$), where  differences or some nonlinear transformation (including deflating and logging) is introduced. $d$ is the number of differences needed to convert a non-stationary time series into a stationary \rev{one. An  ARIMA($p$,$d$,$q$) time series will follow ARMA($p$,$q$) model after $d$ times differences. For example, if a time series $y_t$ follows the ARIMA($p$,$d$,$q$) model, then $\triangle^d$$y_t$ follows the} ARMA($p$,$q$) model, where $\triangle^d$$y_t$ is the sequence of $y_t$ after $d$ times differences. \note{By difference, it also means d lags?}\note{ D times differences are not same with d lags.  A “lag” is a fixed amount of passing time. The $k_{th}$ lag is the time period that happened “k” time points before time i. Lag1(Y2) = Y1 and Lag4(Y9) = Y5}

\paragraph{ARCH Model}

In the ARIMA model, we assume the errors follow the homogeneous Gaussian distribution, while conditional variance is used in Auto-Regressive Conditional Heteroscedasticity (ARCH) model. The ARCH($P$) model has the following structure:
\begin{equation}
\label{ARCH}
    \begin{cases}
      y_t = \mu_t + u_t \\
      u_t = z_t{\sqrt{h_t}}\quad  z_t\sim N(0,1)\\
      h_t = w+\sum_{j=1}^{P} {\lambda_j{u_{t-j}^2}}
    \end{cases}
\end{equation}
where the constant $\mu_t$ is usually assumed to equal the expectation of the time series. The random error $u_t$ is a function of $z_t$ with normal distribution  and the GARCH term $h_t$ (i.e. conditional variance).  $\lambda_j$ is a weight. 

\paragraph{GARCH Model and ARMA-GARCH Model}

The conditional variance functions of some residual time series often have the feature of auto-regression, where the current conditional variance is also affected by the previous conditional variance values. As a generation of the ARCH model, the GARCH($P,Q$) model follows
\begin{equation}
    \begin{cases}
      y_t = \mu_t + u_t \\
      u_t = z_t{\sqrt{h_t}}\quad z_t\sim N(0,1)\\
      h_t = w+\sum_{j=1}^{P} {\lambda_j{u_{t-j}^2}}+\sum_{i=1}^{Q}{\beta_i{h_{t-i}^2}}
    \end{cases}
\end{equation}
where $h_t$ is the conditional variance. GARCH model can be integrated with ARMA model below
\begin{equation}
    \begin{cases}
      y_t = \mu_t + u_t \\
     u_t = \sum_{i=1}^{p} {\alpha_i{u_{t-i}}} + e_t+ \sum_{j=1}^{q} {\theta_j{e_{t-j}}}\\
     e_t = z_t{\sqrt{h_t}} \quad  z_t\sim N(0,1)\\
      h_t = w+\sum_{j=1}^{P} {\lambda_j{e_{t-j}^2}}+\sum_{i=1}^{Q}{\beta_i{h_{t-i}^2}}
    \end{cases}
\end{equation}
to form ARMA($p$,$q$)-GARCH($P$,$Q$) model. If $y_t$ is not stationary, it can be replaced with the $d$ times difference series $\triangle^d$$y_t$  to form the ARIMA($p$,$d$,$q$)-GARCH($P$,$Q$) model.





==> Model_bak.tex <==
\section{Model-driven Learning}
\vspace{-0.10in}
Model based learning aiming to find the appropriate model contained in the data can better explain the relationship between the data and reveal the mechanism of change among the data. At the same time, it can better Calculate and prove the existence and convergence of theoretical errors and has good analytical properties. Taking financial daily stock data as an example. The financial stock is keep changing over time. For the daily stock data such as daily open price, close price, maximum price and minimum price, it will always change but have some relationships with the former days. For example, the daily close price in day $t$ may related with that in day $t-1, t-2…t-10$. However, the influences the previous daily close prices have on day $t$ may be different. $t-1, t-2$ may have the closer relationships than $t-9, t-10$ have to $t$ since $t-1, t-2$ are closer to $t$ than $t-9, t-10$. The task for model-driven learning here is to find and capture the strong relationship among the data in day $t$ and the data in previous days.
\subsection{ARMA Model}
\vspace{-0.05in}
ARMA, the acronym standing for Auto-Regressive Moving Average, is a general model aiming to forecast a stationary time series. ARMA(p,q) model is a combination of Auto-Regressive(AR($p$)) process and Moving Average(MA($q$)) process. $p$ is number of lagged observations for the auto-regression model, which uses the dependencies between an observation and the lagged observations; $q$ is number of lagged forecast residual errors for the moving average model, which uses the dependency between observations and the lagged forecast errors. 
The general expression for AR($p$) model can be written in the following linear form:
\begin{equation}
				y_t = \mu + \alpha_1{y_{t-1}}+\alpha_2{y_{t-2}}+...+\alpha_p{y_{t-p}}
\end{equation}
Where $y_t$ is a stationary time series, $c$ is a constant, $\alpha_1,\alpha_2,...\alpha_p$ are the auto-correlation coefficients at lags 1,2…$p$, $e_t$ are residuals that are Gaussian white noises series with mean zero and variance $\sigma_t$.

Moving average(MA($q$)) model improves the time series prediction through forecasting the lagged values of the errors, which can be written in the following form:
\begin{equation}
	y_t = \mu + e_t+\theta_1{e_{t-1}}+\theta_2{e_{t-2}}+....+\theta_q{e_{t-q}}
\end{equation}
Where $\mu$ is the expectation of $y_t$(usually assumed equal to zero), $\theta$ terms are the weights for prior stochastic term in time series.$e_t$ are often assumed to follow Gaussian white noises with mean zero and variance $\sigma_t$. 
Combining AR($p$) and MA($q$) models, one can get the ARMA($p$,$q$) model as follow:
\begin{equation}
   y_t = \mu + \sum_{i=1}^{p} {\alpha_i{y_{t-i}}} + e_t+ \sum_{j=1}^{q} {\theta_j{e_{t-j}}}
\end{equation}

\subsection{ARIMA Model}
\vspace{-0.05in}
Auto-Regressive Integrated Moving Average(ARIMA) model is a generalized model of ARMA($p$,$d$,$q$). ARIMA($p$,$d$,$q$) model can deal with the non-stationary time series data via differences or some nonlinear transformation including deflating and logging. $d$ is the number of differences needed to convert a non-stationary time series into a stationary. A time series following ARIMA($p$,$d$,$q$) model is equivalent to follow ARIMA($p$,$d$,$q$) model after d times differences for this series. 

\subsection{ARCH Model}
\vspace{-0.05in}
In the ARIMA model, we assume the errors follow the homogeneous Gaussian distribution; while in Auto-Regressive Conditional Heteroscedasticity (ARCH) model. In the ARCH model, the assumption of homogeneity of variance is no longer used, but conditional variance is used to build the model. The ARCH(P) model has the following structure:
\begin{equation}
    \begin{cases}
      y_t = \mu_t + u_t \\
      u_t = z_t{\sqrt{h_t}}\quad  z_t\sim N(0,1)\\
      h_t = w+\sum_{j=1}^{P} {\lambda_j{u_{t-j}^2}}
    \end{cases}
\end{equation}
where $\mu_t$ is the constant term(usually assumed equal to the expectation of the time series), $u_t$ is the random error terms at time t, $z_t$ is a normal variable, $h_t$ is the GARCH term, which is also called conditional variance, $u_{t-j}$ is the random error at time $t-j$ and $\lambda_j$ is the corresponding weight. 

\subsection{GARCH Model}
\vspace{-0.05in}
Further, in reality, the conditional variance functions of some residual time series have the feature of auto-regression. Namely, the current conditional variance is also affected by the previous conditional variance values. Therefore, a generalized ARCH model, the GARCH model developed by Engle and Bollerslov, is  proposed to model the time series. The GARCH(P,Q) model has the following formulation.
\begin{equation}
    \begin{cases}
      y_t = \mu_t + u_t \\
      u_t = z_t{\sqrt{h_t}}\quad z_t\sim N(0,1)\\
      h_t = w+\sum_{j=1}^{P} {\lambda_j{u_{t-j}^2}}+\sum_{i=1}^{Q}{\beta_i{h_{t-i}^2}}
    \end{cases}
\end{equation}
Where $h_{t-i}$ is the conditional variance at time $t-i$.
GARCH model can be integrated with ARMA model, that is:
\begin{equation}
    \begin{cases}
      y_t = \mu_t + u_t \\
     u_t = \sum_{i=1}^{p} {\alpha_i{u_{t-i}}} + e_t+ \sum_{j=1}^{q} {\theta_j{e_{t-j}}}\\
     e_t = z_t{\sqrt{h_t}} \quad  z_t\sim N(0,1)\\
      h_t = w+\sum_{j=1}^{P} {\lambda_j{e_{t-j}^2}}+\sum_{i=1}^{Q}{\beta_i{h_{t-i}^2}}
    \end{cases}
\end{equation}
The model above is called ARMA($p$,$q$)-GARCH($P$,$Q$) model. If $y_t$ is not stationary, replace $y_t$ with its $d$ times difference series $\triangle^d$,$y_t$ and get ARIMA($p$,$d$,$q$)-GARCH($P$,$Q$) model.





==> comment_table.tex <==
\begin{table}[]
\caption{\label{tab7} Metrics Analysis for data set 2: one week test set}
\vspace{-5pt}
\footnotesize
\begin{tabular}{|c|c|c|c|c|}
\hline
 & MSE & RMSE & MAE & MAPE \\ \hline
AG & 156.926155 & 12.527017 & 10.131694 & 0.566243 \\ \hline
LSTM & 323.919643 & 17.997768 & 16.234742 & 0.904311 \\ \hline
SVR & 470.895402 & 21.700124 & 18.116079 & 0.999655 \\ \hline
\begin{tabular}[c]{@{}c@{}}AG-\\ LSTM\end{tabular} & 108.321137 & 10.407744 & 8.024106 & 0.448959 \\ \hline
\begin{tabular}[c]{@{}c@{}}AG-\\ SVR\end{tabular} & 137.932795 & 11.744479 & 8.918046 & 0.498408 \\ \hline
\end{tabular}
\vspace{-10pt}
\end{table}


\begin{table}[]
\caption{\label{tab6} Metrics Analysis for data set 2: whole test set}
\vspace{-5pt}
\footnotesize
\begin{tabular}{|c|c|c|c|c|}
\hline
 & MSE & RMSE & MAE & MAPE \\ \hline
AG & 410.955999 & 20.272050 & 14.447173 & 0.808469 \\ \hline
LSTM & 514.056597 & 22.672816 & 16.812532 & 0.938494 \\ \hline
SVR & 518.241072 & 22.764909 & 16.192336 & 0.900932 \\ \hline
\begin{tabular}[c]{@{}c@{}}AG-\\ LSTM\end{tabular} & 408.589274 & 20.213591 & 13.786998 & 0.772074 \\ \hline
\begin{tabular}[c]{@{}c@{}}AG-\\ SVR\end{tabular} & 403.106978 & 20.077524 & 14.226647 & 0.796801 \\ \hline
\end{tabular}
\vspace{-5pt}
\end{table}

\begin{table}[]
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 &  & MSE & RMSE & MAE & MAPE \\ \hline
 & AG & 287.66 & 16.96 & 13.92 & 0.78 \\ \cline{2-6} 
Test Set 3 & LSTM & 440.38 & 20.99 & 17.34 & 0.97 \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}c@{}}LSTM-\\ GARCH\end{tabular} & \textbf{285.41} & \textbf{16.89} & \textbf{13.70} & \textbf{0.77} \\ \hline
 & AG & 238.25 & 15.44 & 12.39 & 0.70 \\ \cline{2-6} 
Test Set 4 & LSTM & 367.18 & 19.16 & 15.71 & 0.88 \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}c@{}}LSTM-\\ GARCH\end{tabular} & \textbf{231.80} & \textbf{15.22} & \textbf{11.95} & \textbf{0.67} \\ \hline
\end{tabular}
\end{table}

==> cs_math.tex <==
% Math symbol definitions
\newcommand{\csobssymb}{z}
\newcommand{\csobssignal}[1][]{\ensuremath{\mathbf\csobssymb_{#1}}\xspace}
\newcommand{\csmeassymb}{y}
\newcommand{\csmeas}[1][]{\ensuremath{\mathbf\csmeassymb_{#1}}\xspace}
\newcommand{\cssparsevecsymb}{x}

\newcommand{\csksparsesymb}{d}
\newcommand{\csksparse}[1][]{\ensuremath{\mathbf \csksparsesymb_{#1}}\xspace}

\newcommand{\csidenmtxsymb}{I}
\newcommand{\csidenmtx}[1][]{\ensuremath{\mathbf \csidenmtxsymb_{#1}}\xspace}

\newcommand{\csidenerrmtxsymb}{I_e}
\newcommand{\csidenerrmtx}[1][]{\ensuremath{\mathbf \csidenerrmtxsymb_{#1}}\xspace}

\newcommand{\cssparsevec}[1][]{\ensuremath{\mathbf \cssparsevecsymb_{#1}}\xspace}
\newcommand{\cssparsevecvarsymb}{u}
\newcommand{\cssparsevecvar}[1][]{\ensuremath{\mathbf \cssparsevecvarsymb_{#1}}\xspace}
\newcommand{\cssparsevecvaraltsymb}{v}
\newcommand{\cssparsevecvaralt}[1][]{\ensuremath{\mathbf \cssparsevecvaraltsymb_{#1}}\xspace}
\newcommand{\cssparsevecest}[1][]{\ensuremath{\hat{\mathbf \cssparsevecsymb}_{#1}}\xspace}
\newcommand{\cssparsevecshift}[1][]{\ensuremath{\tilde{\mathbf \cssparsevecsymb}_{#1}}\xspace}
\newcommand{\csdict}[1][]{\ensuremath{\bm\Psi_{#1}}\xspace}
\newcommand{\csmeasmtx}[1][]{\ensuremath{\bm\Phi_{#1}}\xspace}
\newcommand{\cssysmtx}[1][]{\ensuremath{\mathbf A_{#1}}\xspace}
\newcommand{\circshift}[3]{\ensuremath{#1_{\circlearrowright(#2,#3)}}}
\newcommand{\circshiftvec}[2]{\ensuremath{#1_{\circlearrowright#2}}}
\newcommand{\diag}{\operatorname{diag}}

\newcommand{\cshmtx}[1][]{\ensuremath{\mathbf H_{#1}}\xspace}
\newcommand{\cserrhmtx}[1][]{\ensuremath{\mathbf{\tilde H}_{#1}}\xspace}
\newcommand{\cshmtxerr}[1][]{\ensuremath{\mathbf E_{#1}}\xspace}
\newcommand{\csdmtx}[1][]{\ensuremath{\mathbf D_{#1}}\xspace}
\newcommand{\cserrmeas}[1][]{\ensuremath{\mathbf{\tilde y}_{#1}}\xspace}
\newcommand{\cserrmeasmtx}[1][]{\ensuremath{\bm{\tilde \Phi}_{#1}}\xspace}

\newcommand{\csherrvec}[1][]{\ensuremath{\mathbf e_{#1}}\xspace}
\newcommand{\cssigmtx}[1][]{\ensuremath{\mathbf Z'_{#1}}\xspace}

\newcommand{\noisesymb}{n}
\newcommand{\noise}[1][]{\ensuremath{\mathbf \noisesymb_{#1}}\xspace}
\newcommand{\qnoisesymb}{q}
\newcommand{\qnoise}[1][]{\ensuremath{\mathbf \qnoisesymb_{#1}}\xspace}
\newcommand{\rnoisesymb}{r}
\newcommand{\rnoise}[1][]{\ensuremath{\mathbf \rnoisesymb_{#1}}\xspace}

\DeclareMathOperator{\E}{\mathbb E}
\makeatletter
\newcommand{\expectation}[1]{%
  \@ifnextchar[{\expectation@i{#1}}{\expectation@j{#1}}%]
}
\def\expectation@i#1[#2]{%
  \ensuremath{\E_{#2}\left[#1\right]}\xspace%
}
\def\expectation@j#1{%
  \ensuremath{\E\left[#1\right]}\xspace%
}
\makeatother
\newcommand{\transpose}{\ensuremath{^\mathrm{T}}}


==> old_tex/Dynamic_050620_pre-revamp.tex <==
%\section{Learning of Dynamics Process }
\section{\textcolor{red}{Learning Out-of-Equilibrium Dynamics} }

\begin{wrapfigure}[9]{r}{2.9in}
  \vspace{-30pt}
  \begin{center}
\includegraphics[width=2.9in]{images/speckle}
  \end{center}
  \vspace{-20pt}
  \caption{\footnotesize Time-series of speckle pattern.}
\label{speckle}
  \vspace{-10pt}
\end{wrapfigure}

If the distribution of matter or disorder within a sample fluctuates in time, the X-ray speckle pattern generated by coherent scattering from the sample will also fluctuate. XPCS relates fluctuations
in the speckle pattern to the dynamics within the sample via the normalized intensity-intensity correlation
function:

\begin{equation}
g_2(\vec{Q},t)=\frac{\mathopen{<}I(\vec{Q},t')I(\vec{Q},t'+t) \mathclose{>}}{\mathopen{<}I(\vec{Q})\mathclose{>}^2}= 1+\beta\mathopen{<}E(\vec{Q},0)E(\vec{Q},t)\mathclose{>}^2/I^2=1+\beta\abs{f(\vec{Q},t)}^2,
\label{g2}
\end{equation}
where $\beta$ is the optical contrast, $f(Q,t)$ is the normalized intermediate scattering function (ISF) that measures the density fluctuations, \textcolor{red}{$t$ is the lag time, and $\vec{Q}$ is the scattering vector (wavevector-transfer)}.
 %and can also provide connections with theoretical calculations of material properties.
% Non-equilibrium dynamics can be probed by using a two-time correlation function $g_2(\vec{Q},t_1, t_2)$.
% ISF is found to be able to follow various forms, such as $e^{-D(Q)Q^2t}$ with $D(Q)$ a length scale dependent diffusion constant, a double-exponential decay of the form $f(Q,t) = (1 - \alpha)e^{−\Gamma_1 t} + \alpha e^{−\Gamma_2 t}$ with $−\Gamma_1$ the short-time decay constant and $−\Gamma_2$ the long-time decay constant, or a stretched exponential of the form $e^{-(\Gamma_1 t)^v}$ where $v$ is a stretching factor.




%Intensity correlation has been widely applied in along with materials scanning with XPCS.
%The dynamic structure factor $g_2$ provides the information about how a material responds to perturbations close to equilibrium.

\begin{wrapfigure}[13]{r}{1.9in}
  \vspace{-30pt}
  \begin{center}
\includegraphics[width=1.9 in]{images/2tc}
  \end{center}
  \vspace{-20pt}
  \caption{\footnotesize 2-time Correlation Function in out-of-equilibrium system}
\label{2tc}
  \vspace{-20pt}
\end{wrapfigure}

%The time auto correlation functions of the speckle fluctuations (Fig.~\ref{speckle}) reveals the  information of the density correlations in the sample and their time dependencies.
Fig.~\ref{speckle} shows the time series of speckle pattern. The normalized intensity-intensity  correlation function $g_2$ is widely applied to quantify the sample dynamics.  When the system is under equilibrium, $g_2$ in Equ.~\ref{g2} depends only on the time difference $t$, but not the sample “age” $t'$. The one-time correlation functions are related to the dynamic structure factor of the system and provide information such as the \sout{time and spatially dependent} relaxation time of the nanoscale dynamics within \sout{ the nano-composite system} 
\textcolor{red}{a nanocomposite at a given age}
.  
\textcolor{blue}{[MF: mentioning ``time- and spatially dependent'' in the preceding sentence is distracting and confusing. Time or age dependence will be covered by the following sentence. Leave the spatial heterogeneity to the following section.]}
When the system is not in equilibrium, however, two-time correlation function (2TCF) $g_2(\vec{Q},t_1, t_2)$ will be used (Fig~\ref{2tc}), which can be evaluated as \sout{aged}
\textcolor{red}{evolving or age-dependent} one-time correlation functions, 
\textcolor{red}{with each} corresponding to a specific time point in the experiment.




 %As the internal structure or the environment of the materials vary, it will also impact the parameters of the model. In addition, the actual measurement data often deviate from the theoretical model.

 Exponential-based models such as Kohlrausch function~\cite{Kohlrausch} and double decay function are commonly applied to represent $g_2$ function\sout{, where the parameters are time independent}. \textcolor{blue}{[MF: Too much detail without context; unclear what ``parameters'' refer to; ``time independent'' applies only to equilibrium cases. \textbf{Bring Eq. 2 up here}.]} \sout{Despite} 
 \textcolor{red}{Although} the models provide a good guidance on the pattern of $g_2$, the actual \textcolor{red}{model-}parameter value \textcolor{red}{(e.g., $\alpha$ in Eq. 2)} could change over time during a \sout{dynamic} 
 \textcolor{red}{non-equilibrium}
 process, and can be impacted by materials type and factors such as temperature and concentration. Simply modeling a process with a fixed form or parameter will be subject to failure \textcolor{blue}{[MF: maybe ``prone to failure'' is more appropriate.]}. In addition, the data values from actual measurements often deviate from the theoretical model. It is crucial to better track the dynamics of materials to more accurately predict the evolution \sout{process}
 \textcolor{red}{behavior}, classify the materials
 \textcolor{red}{dynamics}, and guide for more efficient experiment\textcolor{red}{s}.




%In light of the problems, in this project, we propose to investigate along two research thrusts: 1) Model driven data aware machine learning to accurately track the evolution of the dynamic structure factor, and 2) Automatic experiment with multi-dimensional sparse measurements.

\begin{wrapfigure}[9]{r}{1.6in}
  \vspace{-25pt}
  \begin{center}
\includegraphics[width=1.6 in]{images/Model_Data.png}
  \end{center}
  \vspace{-20pt}
  \caption{\footnotesize Model-driven data-aware learning of dynamics.}
\label{mdal}
  \vspace{-20pt}
\end{wrapfigure}

\textcolor{blue}{[MF: In Fig.~\ref{mdal}, replace ``(e.g. Intensity correlation'' with ``e.g., $g_{2}$ function''.]}

%However, for the non-equilibrium system like Gaseous or liquid systems, everything is changing over time. The inner particles of the samples keep doing the Brownian motions and sometimes fluctuate a lot.
 To better understand the dynamics of materials, we would like to explore a {\em model-driven data-aware machine learning} method to track the evolution of the dynamic structure factor $g_2$. To explain our method,  we have $g_2$  represented with a Kohlrausch function as an example, where  a stretched ($0<\alpha<1$) or compressed ($\alpha>1$) exponential-based model is applied:
%\begin{equation}
%g_2(\vec{Q},t) = 1+ \beta \abs{f(\vec{Q},t)}^2 = 1 + \beta e^{-2{(\Gamma(\vec{Q}) t)}^\alpha}, \hspace{0.01in} \Gamma(\vec{Q}) = D_0 q^2.
%\end{equation}
\begin{equation}
g_2(\vec{Q},t) = 1+ \beta \abs{f(\vec{Q},t)}^2 = 1 + \beta e^{-2{(t/\tau_{0}(\vec{Q}))}^\alpha}, %\hspace{0.01in} \Gamma(\vec{Q}) = D_0 q^2.
\end{equation}
%\begin{equation}
%\Gamma(\vec{Q}) = D_0 q^2
%\end{equation}
%
\textcolor{blue}{[MF: Note Fig. 2 was modified.]}
\textcolor{red}{where $\tau_{0}(\vec{Q})$ is the characteristic time scale of the relevant dynamics (e.g., for Brownian dynamics, $\tau_{0} \sim q^{-2}$ with $q = |\vec{Q}|$),}
\sout{Both the  momentum transfer coefficient $q$}
%and $\alpha$ is a stretched or compressed exponential
\sout{and $\alpha$  can be a function of the time $t$} 
 \textcolor{red}{and $\alpha$ can vary with age $t_{age}$}. ML-based methods have proven to be powerful tools to learn the time-varying parameters. Nikravesh~\cite{Nikravesh1996Model} demonstrates that neural networks in conjunction with recursive least squares can be used to effectively learn the parameter of a model for the nonlinear time variant processes. Applying the update method to the non-isothermal continuous stirred tank reactor with time-varying parameters achieves good performance 
 \textcolor{blue}{[MF: What does non-isothermal...reactor have anything to do with ML/NN here? Good performance in/of what? I think the preceding sentence can be removed.]}. Even with the learning of model parameters,  actual measured data still often deviate from the theoretical model. Rather than only relying on the model, to more accurately represent the $g_2$ function, we propose to explore  a {\em model-driven data-aware}  method by concurrently exploiting the model-based learning and pure data driven learning with a neural network (Fig~\ref{mdal}). More specifically, we can first apply
the exponential-based model with time-varying parameters {\em learnt} to fit the model part. We then compute the difference between the model and the actual data measured for training. If the loss is beyond some preset acceptable threshold, we will introduce a suitable neural network method to learn the difference part. In the actual application, the trained exponential-based model and  network will be applied to quickly predict the dynamic process.
%Finally, combining the two part to get more accurate results.
We expect that our proposed method can fully take advantage of the existing $g_2$ models to approximate the dynamic process, and the emerging ML/DL methods 
\textcolor{blue}{[MF: DL is undefined. Just replace ``ML/DL'' with ``deep learning''?]} to capture the non-linear components of the data. Compared to pure data driven machine learning, the incorporation of the  model part helps better interpret the overall process, and greatly reduce the training time.
%The advantage of this method is it can give full play to the ability of analysis based on the model and the ability to process non-linear information based on the drive of the data. This method is not only improving the fit prediction but increase the interpretation of the model.
This method is general and can be  extended to many application fields.



%As a second method(Fig~\ref{mdal}b), we would like to apply a neural network to find the relationship between the intensity and quantified dynamic fluctuation inside the materials by learning the evolution of the intensity directly,  where the intensity measured at a time slice is a multi-dimensional function itself. The correlation of intensity can be calculated  to find the dynamics of the materials. As the intensity at different time slices will form a time serials, a neural network such as RNN, LSTM and GRU  can be used to capture the change of the intensity and make a good prediction of the dynamic process.
%When data is lacking, this approach can help us get more  predicted intensity, which can be feed into the previous DNN model for training.



%instead of intensity-intensity correlation function to acquire the fluctuations in the speckle pattern, we propose a new method to capture the intensity change and specify the dynamic process of materials. In our proposed method, we use Neural Network to find the relationship between intensity and quantified dynamic fluctuation inside the materials.




==> old_tex/Intro_050620_pre-revamp.tex <==
\section{Introduction}
\vspace{-0.15in}

%Long-term monitoring is often needed for surveillance and system management. For example, radar sensors can be placed over rooftops to protect against rogue drones from approaching the surrounding area.
%A network of drones could be applied to monitor a domain to support applications such as coastal patrol and mine protection.

Modern synchrotrons enable in-situ/operando experiments across a wide range of disciplines like physics, chemistry and material science. Commonly the phase space of such an experiment is larger than the phase space that can be simultaneously sampled. While AI and ML based autonomous experiments are drawing attentions for efficiently sampling the phase space, especially in ex-situ experiments (i.e. static samples), 
experiments covering out-of-equilibrium phenomena present an additional challenge, due to the time-dependent nature of the sample. Many out-of-equilibrium processes are irreversible, i.e. each point in time is only available once for a measurement for any given sample and adding a different measurement at the same time point requires re-creating the sample conditions or the sample itself. In such a situation, it is of paramount importance to conduct measurements following an ‘Optimum Data Collection Trajectory’ (ODCT) to maximize the value of data collected during the continuous evolution of the sample.
%, while potentially employing different experimental techniques in a multi-modal approach.

In this seed project, we propose to develop fundamental techniques that can facilitate more efficient and intelligent experiments. We will explore emerging machine learning (ML) and sparse data sampling techniques for accurately modeling out-of-equilibrium processes and finding ODCT. As a specific use-case, we will apply X-ray Photon Correlation Spectroscopy (XPCS) to Additive Manufacturing (‘3D printing’) of polymer nanocomposites. 
\textcolor{blue}{[MF: Cite Lutz' recent papers on XPCS/3D printing/nanocomposites here: doi: 10.1080/08940886.2019.1582285 ; doi: 10.1021/acs.langmuir.9b00766 ; doi: 10.1063/1.5141488 ; doi: 10.1016/j.mtphys.2020.100220 ]}
Our research will fall into two thrusts: 1) Model-driven data-aware machine learning to accurately track the 
evolving dynamics at a given material location, and 2) Active sparse scanning for efficiently probing spatially-varying dynamics that occurs in 3D printing processes.
%Determining ODCT with multi-dimensional sparse measurements.

 Beyond the specific use case, the principle of ODCTs will be applicable to a wide range of experiments, such as spectroscopy imaging with X-ray nanoprobes, and can be generalized to many out-of-equilibrium experiments where the parameter phase space is larger than what can be probed simultaneously.



%X-ray diffraction is an important tool as structural probe for condensed matter on atomic length scales. Since its early beginning, it allows the structural determination of a wide variety of materials. Inherent in conventional X-ray diffraction experiment is an ensemble averaging process over the illuminated volume of the sample. Such an averaging process is often desirable as it allows atomic-scale quantities to be measured over a region of micro- to millimeters with a great statistic precision. However, the incoherent averaging process leads to a loss of information, which is not desirable when samples are non-periodic or evolve over time.

%Understanding and creating new materials increasingly require measurements of not only the time averaged or instantaneous properties of the material but also its kinetic and dynamic behavior. X-ray photon correlation spectroscopy (XPCS) provides such information at the nanoscale and below by characterizing fluctuations in condensed matter across a broad range of length and time scales. The spatiotemporal range provided by XPCS today with the ongoing development of diffraction-limited storage rings will enable studies \cite{doi:10.1146/annurev-matsci-070317-124334} of nucleation and precipitation and growth, coarsening, eutectic solidification and spinodal decomposition, dealloying, dewetting, solute trapping, electro migration, and many other processes that are vital for understanding fundamentals of materials phase transformation, materials processing and synthesis.

%\vspace{0.06in}
%\noindent{{\bf{Problem 1:} } If the distribution of matter or disorder within a sample fluctuates in time, the X-ray speckle pattern generated by coherent scattering from the sample will also fluctuate. XPCS relates fluctuations in the speckle pattern to the dynamics within the sample via the normalized intensity-intensity correlation function:

%\begin{equation}
%g_2(\vec{Q},t)=\frac{\mathopen{<}I(\vec{Q},t')I(\vec{Q},t'+t) \mathclose{>}}{\mathopen{<}I(\vec{Q})\mathclose{>}^2}= 1+\beta\mathopen{<}E(\vec{Q},0)E(\vec{Q},t)\mathclose{>}^2/I^2=1+\beta\abs{f(\vec{Q},t)}^2,
%\label{g2}
%\end{equation}
%where $\beta$ is the optical contrast, $f(Q,t)$ is the normalized intermediate scattering function (ISF). The ISF provides a measure of density fluctuations within a material. Knowledge of the dynamic structure factor $g_2$ provides the information about how a material responds to perturbations close to equilibrium and can also provide connections with theoretical calculations of material properties. Non-equilibrium dynamics can be probed by using a two-time correlation function $g_2(\vec{Q},t_1, t_2)$. ISF is found to be able to follow various forms, such as $e^{-D(Q)Q^2t}$ with $D(Q)$ a length scale dependent diffusion constant, a double-exponential decay of the form $f(Q,t) = (1 - \alpha)e^{−\Gamma_1 t} + \alpha e^{−\Gamma_2 t}$ with $−\Gamma_1$ the short-time decay constant and $−\Gamma_2$ the long-time decay constant, or a stretched exponential of the form $e^{-(\Gamma_1 t)^v}$ where $v$ is a stretching factor.

%For a material, it needs to determine which model follow. Despite the models provide a good guidance for the trend of ISF and $g_2$, the actual parameter value could change over time during a dynamic process, and can be impacted by materials type and factors such as temperature and concentration. Simply modeling a process with a fixed form or parameter will be subject to failure. In addition, the data values from actual measurements often deviate from the theoretical model. It is crucial to better track the dynamics of materials to more accurately predict the evolution process, classify the materials, and guide for more efficient experiment.

%to more accurately follow the evolution process, classify the materials, and better guide the experiment.
%\vspace{0.06in}
%\noindent{{\bf{Problem 2:} } In a dynamic process, the model parameter may evolve over time, and the actual data often deviate from the model. In addition, the structure and properties of the majority of materials for industry and research depend on a large number of material composition and processing parameters. This makes it essential to explore and understand the composition-processing-structure-property relations of materials in their associated multi-dimensional parameter spaces. Each space is a combination of the parameters that affect an experiment, including synthesis and processing conditions, material composition, and environmental conditions during the experiment. Traditionally, the parameters of the experiment are changed  manually and interactively, where the next measurement parameters are determined based on the analysis of the recent and all prior results. This process is not only time and resource consuming, but is also insufficient or even infeasible to explore the vast, high-dimensional parameter spaces that underlies the complex materials.

%In light of the problems, in this project, we propose to investigate along two research thrusts: 1) Model driven data aware machine learning to accurately track the evolution of the dynamic structure factor, and 2) Automatic experiment with multi-dimensional sparse measurements.

%\vspace{0.06in}
%\noindent{{\bf External funding opportunities:}} Our research methods are general. Besides its application in materials scanning with XPCS, it can be extended to apply in many scientific fields that involve the modeling of time evolving system states as well as low cost yet fine grade measurements. We expect the collaboration of SBU and BNL will attract additonal funding from DOE, NSF and DOD.





